InfoGuard: A Design and Usability Study of User-Controlled Application-Independent Encryption for Privacy-Conscious Users

Billions of secure messaging users have adopted end-to-end encryption (E2EE). Nevertheless, challenges remain. Most communication applications do not provide E2EE, and application silos prevent interoperability. Our qualitative analysis of privacy-conscious users' discussions of E2EE on Reddit reveals concerns about trusting client applications with plaintext, lack of clear indicators about how encryption works, high cost to switch apps, and concerns that most apps are not open source. We propose InfoGuard, a system enabling E2EE for user-to-user communication in any application. InfoGuard allows users to trigger encryption on any textbox, even if the application does not support E2EE. InfoGuard encrypts text before it reaches the application, eliminating the client app's access to plaintext. InfoGuard also incorporates visible encryption to make it easier for users to understand that their data is being encrypted and give them greater confidence in the system's security. The design enables fine-grained encryption, allowing specific sensitive data items to be encrypted while the rest remains visible to the server. Participants in our user study found InfoGuard usable and trustworthy, expressing a willingness to adopt it.

==> Evaluation_old.tex <==
\section{Evaluation}

\tarun{Need to revise this section. Lets discuss these properties an alternates names on zoom. Then, I'll do first pass on improving this.}

% \ks{This isn't the kind of security an usability evaluation we sometimes see, so I would emphasize that we compared the security, scalability, and usability of \sysname to other E2EE systems according to a set of metrics in these areas as shown in the figure. It isn't intended to be exhaustive. Some will recognize this kind of comparison to many prior works since the Quest pw paper.}


This section provides a comparative analysis of \sysname with other end-to-end encryption (E2EE) systems based on a set of predefined metrics related to security, scalability, and perceived usability. The comparison is presented in Table~\ref{table:system_comparison}, but it is not meant to be exhaustive. Our focus is on the properties that we deem essential for promoting the widespread adoption of E2EE, based on the results of our analysis of Reddit user feedback.

% In this section, we assess the effectiveness of \sysname in terms of security, scalability, and perceived usability. Given that user satisfaction and adoption are closely tied to perceived usability, we emphasize evaluating this aspect. To evaluate \sysname's performance, we compare it with other E2EE systems using different metrics as described in Table~\ref{} \tarun{Describe how we choose metrics?}. 
% We also conduct a performance analysis of \sysname to provide a comprehensive understanding of its capabilities.

\input{comparison_table_old}


\subsection{Security}
\textit{Server access:} In an E2EE system, (1) preventing data access from a server is a critical requirement. While all the E2EE systems evaluated in our analysis prevent data access from a passive server, FlyByNight stores the user's private key encrypted with a password on the server, which can be brute-forced to retrieve the private key. As passwords are often weak, FlyByNight only received a half circle in our evaluation. Two common active attacks a server can execute are distributing fake keys to execute MITM for the client and inserting malicious code on their client app. 
\ks{Should fake key attack be a column? Are all of these apps using a centralized key server to distribute public keys and all vulnerable to this attack?} 
\tarun{Yes! All of these are vulnerable to fake key attacks. some of them do not even talk about key distribution and says any key distribution is used that is considered more secure.}
The fake key distribution attacks can be detected or prevented using secure key distribution techniques such as CONIKS~\cite{melara2015coniks}, SEEMLESS~\cite{chaseseemless}, and KTACA~\cite{yadav2022automatic}. These secure key distributions can be applied to any E2EE system, including PGP and S/MIME, to detect the distribution of fake key attacks. 


\textit{Passive and active client attacks:} The application can execute two types of attacks on the client side: passive and active. (2) Passive attacks involve reading user text and sending it to the server or having bugs that allow other attackers to access plain text. (3) Active attacks involve the client app trying to access the plaintext when the user does not enter it directly into the app. Browser extension-based and phone-based systems that leverage accessibility APIs prevent only passive attacks by passing only the encrypted text to the target application. In all other systems, the client app has access to plaintext. \sysname, on the other hand, prevents plaintext access from the target app even if it tries to get a   q ccess to the plaintext by executing active attacks.

\textit{No app support required} Encryption protocols such as PGP, S/MIME, and OTR-based protocols require applications to support encryption, thereby limiting user control over what to encrypt and what algorithms to use. Moreover, this also implies that the system's security is spread across multiple applications, making it harder to evaluate the system's overall security. In contrast, application-independent systems allow users to control such aspects of the encryption process and do not require app support to encrypt user content. Moreover, because these application-independent protocols have a centralized implementation, (5) evaluating code security and implementing quick patches becomes significantly easier. 

Most applications implement application-dependent protocols through libraries, which means that analyzing and patching those libraries could fix many applications. Therefore, instead of saying there are no easy ways to evaluate and patch for application-dependent protocols, we say sometimes (denoted by a half circle in the table). 

\ks{This section makes it hard to see what text lines up with the 6 columns. I marked some parts temporarily to show when I could see a column being discussed. For starters, put each item in its own paragraph for clarity.}



\subsection{Scalability}
% \ks{It would help to have a paragraph for each column. I don't understand column 2, and it isn't clear if the first part of the last paragraph is meant to describe it.}
The concept of application independence refers to a system's ability to provide encryption without any necessary action required from the application itself. This functionality makes it easier for users to adopt encryption protocols without waiting for individual applications to update their security measures. A few examples of application-independent end-to-end encryption (E2EE) systems include browser extension-based systems such as Mimesis Aegis, BabelCrypt, and \sysname. 

However, it's important to note that being application independent does not guarantee that a system will work seamlessly with all applications. The system also needs to ensure to not have unscalable dependencies. For instance, browser extension-based E2EE systems and Mimesis Aegis require overlay designs that mimic the original app's graphical user interface (GUI) for every application they want to support. Additionally, they must frequently update the overlay interface as the original app updates its GUI. Babelcrypt automates the GUI mapping process by prompting users to click on text fields for setting purposes.
Nonetheless, a malicious app can use frequent GUI updates to interfere with the system. Mimesis Aegis and Babelcrypt also utilize the accessibility API, which is not intended to implement security protocols and can create issues in adoption because Google Play Store removes all apps that use accessibility APIs for purposes other than accessibility. In contrast, the \sysname system does not require an app's GUI mapping and avoids using restricted APIs. 

\sysname is the only system that provides an API for developers to secure user data on any text field in their applications. The socket API is language-independent, making it easier for a wide range of applications to use without writing and maintaining extensive code. This feature provides developers with flexibility and simplicity in integrating encryption functionality into their applications without worrying about the complexity of the encryption process.



\subsection{Perceived Usability}
% \ks{It would help if the text in this section lined up exactly with the columns in the Table. I don't understand column 2 heading and it isn't clearly in order in the text of this section.}
The usability of a system is a critical factor in determining its adoption and value in the real world. Our analysis of perceived usability includes metrics that go beyond just the user interface (UI) to consider other important properties, such as user trust. 

While most application-based systems encrypt everything a user types in the application, previous research indicates that users prefer only to encrypt sensitive information instead of everything. Additionally, the definition of sensitive data varies among users, and they may choose to encrypt only what they consider to be sensitive. In the \sysname system, users can selectively encrypt text on any app. For example, they can encrypt either the entire email or just one sentence in an email. While phone-based and browser-based systems also allow selective encryption to some extent, they do not provide the fine-grained control that \sysname does, such as encrypting part of an email.



Most end-to-end encryption (E2EE) systems aim to provide transparent encryption to improve the user experience. However, previous research shows that users do not trust a system if everything happens in the background without any visibility. In \sysname, we offer translucency, allowing users to see that plaintext is encrypted and only encrypted text is passed to the application. While complete translucency may not preserve the original app's UX, the UI of the original app remains the same, but users see encrypted text in the original app. Transparency and translucency are opposing properties, allowing a system to choose between visible encryption and preserving the original app's UX. Application-based systems are completely transparent, while phone-based and browser-based systems provide some translucency by showing users a colored dot, different background, or surrounding box. However, users still type plaintext in the app and do not see encryption happening in real-time. \sysname allows users to selectively encrypt their text while offering complete translucency, improving the user's trust and confidence in the system.

\ks{This last paragraph isn't clearly mapped to the last two properties in the table. In general this entire comparison section can probably be made more concise and more clearly aligned so the discussion is column by column. Some of the column labels are lengthy and we should work on shorter alternatives.}








% The requirement of local storage is only because we use Signal protocol here to achieve forward secrecy. If saving space is essential any other encryption protocol such as PGP could be used which stores the encryption keys permanently. 


% What things we break in apps through \sysname: 





% As illustrated in table~\ref{}, \sysname has stronger security properties especially for preventing active attacks from malicious applications.

% Our \sysname runs on the same Operating system as the target application and 



% \paragraph{Usability Issues}
% The presented design (refer to) appends metadata of \tarun{how many?} length to the message while the user is typing. This approach creates two major issues: (1) the ciphertext becomes longer than the plaintext, leading to confusion and misinterpretation of the message, and (2) the metadata updates for every key press, resulting in a cluttered and confusing user interface. Furthermore, the metadata addition makes it difficult for users to modify the plaintext through the application's interface. 


% Security -- Client app access, Server access, Trust on a third party, forward secrecy, Admin/user control on encryption, Easy patches, open source\\
% Scalable -- Application independent, Easy code verification, Easy code patches, \\
% User perception -- Selective encryption, Desktop application?, 
% Usablity -- Put all the usability things we talked about. 



% USABILITY
% 	Original app's UI experience
% 	noticeable encryption (other alternate is see-through encryption)

% SCALABILITY
% 	UI analysis requried for every app
% 	app support not required (This could come under security category too)
% 	encryption support for developers
% 	no non-scalable dependencies in design (For example Mimesis Aegis [33] and Babelcrypt [42] authors leverage
% accessibility services to create transparent overlays. Accessibility services were not meant to be used for any other purposes.)

% SECURITY
% 	Ease of security code patches
% 	Isolation of encryption logic from client app (Alternate: Confidentiality from client app)
% 	forward secrecy





% \subsection{Screenshot by client app}
% X11 -> allows screenshots by client apps. Wayland and windows GUI manager doesn't allow apps to take screenshot.

% https://unix.stackexchange.com/questions/648178/block-screen-sharing

% In the X11 security model every client that can access the X server and isn't restricted by a X server extension is trusted by default and can use queries like XCopyArea or XGetImage to capture the content of every window on the screen. The reasons for this are mostly historical, as the first version of the X11 protocol was released in 1987 and security features were later "bolted on".

% Wayland has a stricter security design. There only the compositor or design ated trusted applications can access the content of other windows.

% \textbf{The X Access Control Extension framework}
% One elaborate solution to block screen sharing would be to write a X server extension module using the X Access Control Extension (XACE). This extension provides hooks for other extension modules to allow fine-grained access control decisions.

% \subsection{Malicious app can execute attacks}
% A malicious app can ask interceptor to encrypt with a fake key. And then they will be able to decrypt it. 

% benefits of writing directly to framebuffer from GUI interface:
%     Enhanced security for graphical user interfaces (GUIs): Writing text to a framebuffer can improve security for GUIs by enabling them to bypass the X Window System, which has been known to be vulnerable to security attacks. By writing text directly to the framebuffer, the application can avoid using X11, which could potentially reduce the number of security vulnerabilities.

%     Mitigation of screen scraping attacks: Screen scraping attacks are a type of attack where an attacker captures information from the screen. By writing text to the framebuffer, the application can make it more difficult for attackers to capture sensitive information from the screen, as it is not stored in a file or elsewhere on the system.






% \subsection{Comparison w/ Other systems}
% PGP, S/MIME
% Mimesis Aegis:
%     apps can take a screenshot
%     apps can create an overlay and get text input

% Babelcrypt
%     no key management. The user or the system does not select the recipient and therefore uses the same key for every client.
%     uses Android Accessibility Framework android


% Prevents server access: Server cannot see plaintext
% Prevents passive client app access: App does not have access to plaintext (if it doesn't try to execute some active attack)
% Prevents active malicious client app access: App does not have access to plaintext, even if try to attack the system
% forward secrecy
% Admin/user control on encryption: is system designed in a way to allow user/admin decide the strength of algorithm if they want to.
% easy security evaluation and patches: How hard will it be to evaluate the code and apply security patches on the system.
% no app support required: Does the system requires application's support for encryption
% Application independent: Does the system uses application specific dependencies in their design such as relying on app's GUI.
% no non-scalable dependencies in design: Does a system has any requirements that will be hard to scale such as accessibility API used by Mimesis Aegis.
% centralized language independent APIs for developers: Support for developers to enable encryption if they want on their app
% Works for apps outside browser: Not browser specific
% Selective encryption: User can choose when or what to encrypt
% Trust due to encryption system type: Users trust the system apps more than webpages.
% Visible encryption indication: Can users see how and when their data is encrypted.

==> Evaluation_very_old.tex <==
\section{Evaluation}

% \ks{This isn't the kind of security an usability evaluation we sometimes see, so I would emphasize that we compared the security, scalability, and usability of \sysname to other E2EE systems according to a set of metrics in these areas as shown in the figure. It isn't intended to be exhaustive. Some will recognize this kind of comparison to many prior works since the Quest pw paper.}


This section provides a comparative analysis of \sysname with other end-to-end encryption (E2EE) systems based on a set of predefined metrics related to security, scalability, and perceived usability. The comparison is presented in Table~\ref{table:system_comparison}, but it is not meant to be exhaustive. Our focus is on the properties that we deem essential for promoting the widespread adoption of E2EE, based on the results of our analysis of Reddit user feedback.

% In this section, we assess the effectiveness of \sysname in terms of security, scalability, and perceived usability. Given that user satisfaction and adoption are closely tied to perceived usability, we emphasize evaluating this aspect. To evaluate \sysname's performance, we compare it with other E2EE systems using different metrics as described in Table~\ref{} \tarun{Describe how we choose metrics?}. 
% We also conduct a performance analysis of \sysname to provide a comprehensive understanding of its capabilities.

\input{comparison_table}


\subsection{Security}
In an E2EE system, (1) preventing data access from a server is a critical requirement. While all the E2EE systems evaluated in our analysis prevent data access from a passive server, FlyByNight stores the user's private key encrypted with a password on the server, which can be brute-forced to retrieve the private key. As passwords are often weak, FlyByNight only received a half circle in our evaluation. Two common active attacks a server can execute are distributing fake keys to execute MITM for the client and inserting malicious code on their client app. 
\ks{Should fake key attack be a column? Are all of these apps using a centralized key server to distribute public keys and all vulnerable to this attack?} 
\tarun{Yes! All of these are vulnerable to fake key attacks. some of them do not even talk about key distribution and says any key distribution is used that is considered more secure.}
The fake key distribution attacks can be detected or prevented using secure key distribution techniques such as CONIKS~\cite{melara2015coniks}, SEEMLESS~\cite{chaseseemless}, and KTACA~\cite{yadav2022automatic}. These secure key distributions can be applied to any E2EE system, including PGP and S/MIME, to detect the distribution of fake key attacks. The app can execute two types of attacks on the client side: passive and active. (2) Passive attacks involve reading user text and sending it to the server or having bugs that allow other attackers to access plain text. (3) Active attacks involve the client app trying to access the plaintext when the user does not enter it directly into the app. Browser extension-based and phone-based systems that leverage accessibility APIs prevent only passive attacks by passing only the encrypted text to the target application. In all other systems, the client app has access to plaintext. \sysname, on the other hand, prevents plaintext access from the target app even if it tries to get access to the plaintext by executing active attacks.

Encryption protocols such as PGP, S/MIME, and OTR-based protocols require applications to support encryption, thereby limiting user control over what to encrypt and what algorithms to use. Moreover, this also implies that the system's security is spread across multiple applications, making it harder to evaluate the system's overall security. In contrast, application-independent systems allow users to control such aspects of the encryption process and do not require app support to encrypt user content. Moreover, because these application-independent protocols have a centralized implementation, (5) evaluating code security and implementing quick patches becomes significantly easier. 

Most applications implement application-dependent protocols through libraries, which means that analyzing and patching those libraries could fix many applications. Therefore, instead of saying there are no easy ways to evaluate and patch for application-dependent protocols, we say sometimes (denoted by a half circle in the table). 

\ks{This section makes it hard to see what text lines up with the 6 columns. I marked some parts temporarily to show when I could see a column being discussed. For starters, put each item in its own paragraph for clarity.}



\subsection{Scalability}
% \ks{It would help to have a paragraph for each column. I don't understand column 2, and it isn't clear if the first part of the last paragraph is meant to describe it.}
The concept of application independence refers to a system's ability to provide encryption without any necessary action required from the application itself. This functionality makes it easier for users to adopt encryption protocols without waiting for individual applications to update their security measures. A few examples of application-independent end-to-end encryption (E2EE) systems include browser extension-based systems such as Mimesis Aegis, BabelCrypt, and \sysname. 

However, it's important to note that being application independent does not guarantee that a system will work seamlessly with all applications. The system also needs to ensure to not have unscalable dependencies. For instance, browser extension-based E2EE systems and Mimesis Aegis require overlay designs that mimic the original app's graphical user interface (GUI) for every application they want to support. Additionally, they must frequently update the overlay interface as the original app updates its GUI. Babelcrypt automates the GUI mapping process by prompting users to click on text fields for setting purposes.
Nonetheless, a malicious app can use frequent GUI updates to interfere with the system. Mimesis Aegis and Babelcrypt also utilize the accessibility API, which is not intended to implement security protocols and can create issues in adoption because Google Play Store removes all apps that use accessibility APIs for purposes other than accessibility. In contrast, the \sysname system does not require an app's GUI mapping and avoids using restricted APIs. 

\sysname is the only system that provides an API for developers to secure user data on any text field in their applications. The socket API is language-independent, making it easier for a wide range of applications to use without writing and maintaining extensive code. This feature provides developers with flexibility and simplicity in integrating encryption functionality into their applications without worrying about the complexity of the encryption process.



\subsection{Perceived Usability}
% \ks{It would help if the text in this section lined up exactly with the columns in the Table. I don't understand column 2 heading and it isn't clearly in order in the text of this section.}
The usability of a system is a critical factor in determining its adoption and value in the real world. Our analysis of perceived usability includes metrics that go beyond just the user interface (UI) to consider other important properties, such as user trust. 

While most application-based systems encrypt everything a user types in the application, previous research indicates that users prefer only to encrypt sensitive information instead of everything. Additionally, the definition of sensitive data varies among users, and they may choose to encrypt only what they consider to be sensitive. In the \sysname system, users can selectively encrypt text on any app. For example, they can encrypt either the entire email or just one sentence in an email. While phone-based and browser-based systems also allow selective encryption to some extent, they do not provide the fine-grained control that \sysname does, such as encrypting part of an email.



Most end-to-end encryption (E2EE) systems aim to provide transparent encryption to improve the user experience. However, previous research shows that users do not trust a system if everything happens in the background without any visibility. In \sysname, we offer translucency, allowing users to see that plaintext is encrypted and only encrypted text is passed to the application. While complete translucency may not preserve the original app's UX, the UI of the original app remains the same, but users see encrypted text in the original app. Transparency and translucency are opposing properties, allowing a system to choose between visible encryption and preserving the original app's UX. Application-based systems are completely transparent, while phone-based and browser-based systems provide some translucency by showing users a colored dot, different background, or surrounding box. However, users still type plaintext in the app and do not see encryption happening in real-time. \sysname allows users to selectively encrypt their text while offering complete translucency, improving the user's trust and confidence in the system.

\ks{This last paragraph isn't clearly mapped to the last two properties in the table. In general this entire comparison section can probably be made more concise and more clearly aligned so the discussion is column by column. Some of the column labels are lengthy and we should work on shorter alternatives.}






\paragraph{\textbf{Limitations of \sysname}}

% As \sysname is application independent, it is not aware of the contexts in which users use encryption in the application. The lack of visibility of applications' input validations where users initiate encryption can cause unexpected behaviors or errors when a user sends a message. For example, if a user starts encryption in a field that asks for a zip code and is expecting a specific length digit input, the application will throw an error. Another example could be a user trying to encrypt the email address in the \textit{TO} field while sending an email. An in-depth user study is needed to analyze users' behavior when they use \sysname across different websites and how its UX can be improved to allow users to understand where they can or cannot use \sysname. Allowing control of encryption to users opens up many research avenues that needs to be addressed. 



One of the limitations of \sysname is that it is application independent and lacks awareness of the contexts in which users initiate encryption in various applications. This lack of visibility can result in unexpected behaviors or errors when a user sends a message. For example, if a user initiates encryption in a field that expects a specific length digit input, such as a zip code field, the application may throw an error. Another example is a user attempting to encrypt an email address in the \textit{TO} field while sending an email. An in-depth user study is needed in the future to analyze users' behaviors when they use \sysname across different websites and how the \sysname can be improved to aware users where they can or cannot use \sysname. Allowing control of encryption to users opens up many research avenues that need to be addressed to make it practical

% The requirement of local storage is only because we use Signal protocol here to achieve forward secrecy. If saving space is essential any other encryption protocol such as PGP could be used which stores the encryption keys permanently. 


% What things we break in apps through \sysname: 





% As illustrated in table~\ref{}, \sysname has stronger security properties especially for preventing active attacks from malicious applications.

% Our \sysname runs on the same Operating system as the target application and 



% \paragraph{Usability Issues}
% The presented design (refer to) appends metadata of \tarun{how many?} length to the message while the user is typing. This approach creates two major issues: (1) the ciphertext becomes longer than the plaintext, leading to confusion and misinterpretation of the message, and (2) the metadata updates for every key press, resulting in a cluttered and confusing user interface. Furthermore, the metadata addition makes it difficult for users to modify the plaintext through the application's interface. 


% Security -- Client app access, Server access, Trust on a third party, forward secrecy, Admin/user control on encryption, Easy patches, open source\\
% Scalable -- Application independent, Easy code verification, Easy code patches, \\
% User perception -- Selective encryption, Desktop application?, 
% Usablity -- Put all the usability things we talked about. 



% USABILITY
% 	Original app's UI experience
% 	noticeable encryption (other alternate is see-through encryption)

% SCALABILITY
% 	UI analysis requried for every app
% 	app support not required (This could come under security category too)
% 	encryption support for developers
% 	no non-scalable dependencies in design (For example Mimesis Aegis [33] and Babelcrypt [42] authors leverage
% accessibility services to create transparent overlays. Accessibility services were not meant to be used for any other purposes.)

% SECURITY
% 	Ease of security code patches
% 	Isolation of encryption logic from client app (Alternate: Confidentiality from client app)
% 	forward secrecy





% \subsection{Screenshot by client app}
% X11 -> allows screenshots by client apps. Wayland and windows GUI manager doesn't allow apps to take screenshot.

% https://unix.stackexchange.com/questions/648178/block-screen-sharing

% In the X11 security model every client that can access the X server and isn't restricted by a X server extension is trusted by default and can use queries like XCopyArea or XGetImage to capture the content of every window on the screen. The reasons for this are mostly historical, as the first version of the X11 protocol was released in 1987 and security features were later "bolted on".

% Wayland has a stricter security design. There only the compositor or design ated trusted applications can access the content of other windows.

% \textbf{The X Access Control Extension framework}
% One elaborate solution to block screen sharing would be to write a X server extension module using the X Access Control Extension (XACE). This extension provides hooks for other extension modules to allow fine-grained access control decisions.

% \subsection{Malicious app can execute attacks}
% A malicious app can ask interceptor to encrypt with a fake key. And then they will be able to decrypt it. 

% benefits of writing directly to framebuffer from GUI interface:
%     Enhanced security for graphical user interfaces (GUIs): Writing text to a framebuffer can improve security for GUIs by enabling them to bypass the X Window System, which has been known to be vulnerable to security attacks. By writing text directly to the framebuffer, the application can avoid using X11, which could potentially reduce the number of security vulnerabilities.

%     Mitigation of screen scraping attacks: Screen scraping attacks are a type of attack where an attacker captures information from the screen. By writing text to the framebuffer, the application can make it more difficult for attackers to capture sensitive information from the screen, as it is not stored in a file or elsewhere on the system.






% \subsection{Comparison w/ Other systems}
% PGP, S/MIME
% Mimesis Aegis:
%     apps can take a screenshot
%     apps can create an overlay and get text input

% Babelcrypt
%     no key management. The user or the system does not select the recipient and therefore uses the same key for every client.
%     uses Android Accessibility Framework android


% Prevents server access: Server cannot see plaintext
% Prevents passive client app access: App does not have access to plaintext (if it doesn't try to execute some active attack)
% Prevents active malicious client app access: App does not have access to plaintext, even if try to attack the system
% forward secrecy
% Admin/user control on encryption: is system designed in a way to allow user/admin decide the strength of algorithm if they want to.
% easy security evaluation and patches: How hard will it be to evaluate the code and apply security patches on the system.
% no app support required: Does the system requires application's support for encryption
% Application independent: Does the system uses application specific dependencies in their design such as relying on app's GUI.
% no non-scalable dependencies in design: Does a system has any requirements that will be hard to scale such as accessibility API used by Mimesis Aegis.
% centralized language independent APIs for developers: Support for developers to enable encryption if they want on their app
% Works for apps outside browser: Not browser specific
% Selective encryption: User can choose when or what to encrypt
% Trust due to encryption system type: Users trust the system apps more than webpages.
% Visible encryption indication: Can users see how and when their data is encrypted.

==> Introduction_2.tex <==
\section{Introduction}
In the modern era of digital communication, secure and private communication is of utmost importance due to the frequent exchange of sensitive data. Transport Layer Security (TLS) is a widely used encryption protocol that provides security for data in transit. While TLS is an effective encryption protocol to prevent \ks{???} user-to-server communication, it is insufficient for user-to-user communication as servers can see plaintext. Therefore, there is an urgent need to provide end-to-end encryption (E2EE) for all user-to-user communication. E2EE encrypts the message contents from the sender's device, and only the intended recipient can decrypt the message, making it difficult for anyone else to intercept, read or modify it. 

While E2EE is crucial for all users, it is especially vital for people living in countries with high levels of censorship and surveillance. For these individuals, secure communication channels are critical to avoid detection and potential punishment. Similarly, organizations that handle sensitive data must maintain compliance with various regulations and standards, such as CCPA, GDPR and HIPAA, to protect users' privacy and avoid legal liabilities. E2EE is an effective way to ensure that confidential information remains secure during transmission, even in case of a security breach on the application servers.
\ks{I am unsure about this paragraph. In extreme cases, won't the presence of E2EE draw attention and repercussions for some people? In the case of HIPAA and GDPR, this is usually focused on user to business communication where the business has to access the sensitive info. So I'm unsure if they are strong motivations for E2EE. We can think about other scenarios that may be more compelling. Have to give this more thought.}\\
\tarun{for censorship: If they use specific E2EE applications then yes. But now they will be using standard applications and will just encrypt their data within that. This makes it hard for organizations or countries because they usually ban apps to prevent access to E2EE, but if users use our system, they cannot ban apps. Yes! I agree they can go one step ahead and take action against anyone who uses E2EE physically. However, the idea here is not to prevent them against every attack possible but to provide users access to E2EE when there is no E2EE app available in their organization or country. They will need to decide on the risk and consequences based on their situation.}\\
\tarun{GDPR is not specific to health information. It applies to any user's personal data and requires it to handle those with privacy. But I agree that they might not need to be E2EE to be compliant with GDPR as of now. "The General Data Protection Regulation is a Regulation in EU law on data protection and privacy in the EU and the European Economic Area. The GDPR is an important component of EU privacy law and of human rights law, in particular Article 8 of the Charter of Fundamental Rights of the European Union."}


\tarun{Putting this paragraph here as an example of motivation.}
In a recent incident in 2022~\cite{dadGoogleBan}, an individual captured visual representations of his ailing son's genitalia, which he subsequently transmitted via his Android phone to a medical practitioner through the messaging system of a healthcare provider. With several medical offices still closed due to the COVID-19 pandemic, consultations were taking place virtually. Unfortunately, Google's artificial intelligence (AI) flagged the aforementioned images as potential instances of child sexual exploitation, resulting in the initiation of a police inquiry and the revocation of all of the father's Google accounts. This episode underscores such enterprises' capacity to access communications across different platforms.


In our study, we analyzed 54 communication platforms that are commonly used for personal and business purposes. Out of these, only five apps were found to have implemented end-to-end encryption (E2EE) by default, and none of these five apps were open source. To gain insight into the reasons for the low adoption of E2EE, we conducted a qualitative analysis of discussions on three prominent subreddits: "privacy," "privacyToolsIO," and "privacyGuides." These subreddits have a combined membership of 1.56 million users. From a pool of 5,298 relevant posts that discuss communication privacy, we randomly selected and coded 200 posts to identify common themes and concerns related to communication privacy.


Our results from Reddit analysis show that although E2EE is a viable solution, the issue lies in the fact that applications, not users, decide when to implement E2EE. Currently, most popular applications, such as Email, Slack, Microsoft Teams, and Discord, still use TLS, making it difficult for users to secure their communication. Moreover, even when the applications implement E2EE, their client apps have access to plaintext, which could lead to unintended leakage due to bugs or intentional breaches. Furthermore, users often do not trust E2EE applications, already mentioned by~\cite{abu2018exploring}, as they cannot visibly distinguish between plaintext communication, TLS encryption, and E2EE. Because of the lack of encryption visibility, users rely on the app developer's words to understand the secure data from their app, which has conflicting interests.



% End-to-end encryption (E2EE) has emerged as a viable solution to this problem. Unlike Transport Layer Security (TLS), which only secures data in transit, E2EE encrypts the message contents from the sender's device and only the intended recipient can decrypt the message. This makes it difficult for anyone else, including service providers and governments, to intercept, read or modify the message. However, despite the growing demand for E2EE, most popular applications still use TLS, leaving users vulnerable to interception and snooping.

To address these issues, we propose a Secure extension for the Input driver (\sysname) that provides the control of the encryption to the users in an application-independent, visible and scalable manner. \ks{From reading the paper I'm seeing that the scalability aspect is entirely captured by the application-independent property. If true, we only need to mention one of them here. I think we lead with application-independent in the title and main properties list and somewhere in the paper clarify this approach scales better than the application-by-application approach.} \tarun{Sounds good to me. Agree that application independence is one property that helps with scalability so we cannot put them together as different properties. For scalability, our system ensures that it does not have non-scalable dependencies in design as shown in Table 3.}\sysname is a user space application with admin privileges that listens to all user's keyboard keypresses directly from the keyboard driver for the trigger to start encryption mode. Users can request encryption on any textbox on any application by pressing the shortcut to enable the encryption mode, even if the application does not support E2EE. After a user initiates encryption mode, \sysname gets an exclusive lock on the keyboard output and encrypts everything before passing the text from the keyboard driver to the windowing system such as Wayland, which is responsible for passing the keypresses to applications. 

% To allow users to see what they type, \sysname creates a secure GUI on the screen where it directly passes the plaintext to display to the users. Users see encrypted text on the target application and the plain text on \sysname's GUI in real-time while they type. This provides users with the ability to verify that the correct information is being entered while maintaining security. 

\sysname creates a secure GUI on the screen to allow users to see the plaintext they are typing in real time. The encrypted text is displayed in the target application, while the plain text is shown on \sysname's GUI. This provides users with the ability to verify that the correct information is being entered while maintaining security. \sysname do not add metadata on the applications' textbox to prevent overloading users with unnecessary information. It intercepts the encrypted text using a MITM proxy and appends the metadata before transmission over the internet. This ensures that users only see relevant information in the application's textbox, while additional metadata is hidden from view.
\ks{This description seems focused on writers, but what about readers? They likely see the full encrypted blob. What do they do to read the plaintext? When should we explain the issue that some applications may struggle with more text than expected (like a zip code field)?.}
\tarun{The encrypted text and associated metadata are presented in their entirety to the recipient within their application. To initiate decryption, the recipient selects the encrypted text and triggers the decryption keyboard shortcut. \sysname then generates a secure graphical user interface (GUI) on the recipient's screen that displays decrypted text.}

\tarun{I propose adding a paragraph with title "limitation" in bold in either the design section (6) or analysis section (8).}

% that it controls shows users a secure GUI that displays the plaintext input and live encrypted text in the application GUI character by character. It adds metadata using a network proxy before transmission over the Internet, which it sets up and activates after a user enables encryption.


Our design provides better security properties than existing E2EE architectures by eliminating the client app's access to plaintext. This ensures that the data remains secure even if the client app is compromised, reducing the risk of privacy breaches and data theft. Additionally, our architecture incorporates visible encryption, making it easier for users to understand that their data is being encrypted and providing them with greater confidence in the system's security. Our design also allows for fine-grained encryption, where specific sensitive data items can be encrypted while the rest remains visible to the server. This granularity is a significant advantage over existing E2EE systems that use an all-or-nothing approach, where the entire message or file is encrypted.




Although our system is primarily designed to cater to vulnerable and technically proficient users, it is not limited to them and can be adopted by the masses. However, it is essential to note that the mass adoption of end-to-end encryption (E2EE) requires improving users' mental models towards it~\cite{renaud2014doesn}. In this regard, \sysname provides a unique visible encryption method to help users better understand the E2EE process and improve their mental models. \sysname is a technically feasible visible encryption system that can be researched further by performing UX tweaks to enhance users' trust, mental model, and overall experience with E2EE.


In summary, our contributions include (1) an analysis of popular apps, (2) an analysis of users' concerns and perceptions that hinder E2EE adoption, and (3) a centralized application-independent E2EE architecture that eliminates the client app's access to plaintext and incorporates visible encryption, providing users with greater confidence in the system's security. Additionally, our design enables fine-grained encryption, allowing specific sensitive data items to be encrypted while the rest remains visible to the server to provide a personalized user experience.

\ks{I'm thinking of how to rephrase the contributions.
(1) an analysis of Reddit users discussing E2EE to determine for adopting or not adopting E2EE tools.
(2) an analysis of popular messaging apps to determine how well they match the preferences for those adopting E2EE.
(3) the design of InfoGuard, an architecture for user-controlled, application-independent E2EE.
(4) a proof-of-concept implementation of InfoGuard,
(5) a comparative analysis of InfoGuard compared to other E2EE tools.
}


x

==> Reddit_analysis_old.tex <==

\section{Reddit analysis}

\tarun{Comment on the ethics issue.}

% To understand the adoption of E2EE, we analyze popular communication tools used in personal and business as shown in~\ref{table_app_anaysis}. 

Despite the relatively long existence of E2EE technology, its adoption remains limited among users. We aim to identify the concerns, challenges, and perceptions that hinder E2EE adoption. By doing so, we answer the following research question that will help us design an effective E2EE system:

\paragraph{\textbf{Research question}} \textit{For users concerned about privacy, what factors influence them to decide whether to use E2EE and which tools to use?}

% \begin{itemize}
% \item [RQ1] What factors impede the widespread adoption of end-to-end encryption (E2EE)?
% \item [RQ2] How do users perceive the effectiveness of current E2EE solutions, and what are their primary concerns or reservations about using them?
% \item [RQ3] What factors influence users' selection of privacy-enhancing apps?
% \item [NewRQ] For users concerned about privacy, what factors influence them to decide whether to use E2EE and which tools to use?
% \end{itemize}

% \ks{Think through these research questions. I find RQ1 and RQ3 are quite simliar. I read the section on RQ3 and it overlaps with concepts in RQ1. Is that really one question? What makes users choose an E2EE app? Even RQ2 talks about open source, and issue in RQ1. And RQ2 is highly relevant to RQ1. Is it simpler to have a single RQ and talk about all of these issues together?}
% \tarun{I would prefer if we combine them. There are some differences. RQ1 tells us why users do not use E2EE and RQ3 tells us if they choose to secure their communication, how they decide what app to use among so many available. The critical difference in RQ3 the user is already motivated and willing to use the app that they think is most secure. However, I agree that even if a user is willing to secure their connection there are some factors that lead them to prevent using E2EE and it would fall under RQ1. I propose we have one RQ \ie RQ1 - "What factors impede the widespread adoption of end-to-end encryption (E2EE)?"}
% \ks{See if you like the newRQ above, and revise this entire section to have one RQ and consolidate redundant ideas. Since this is only part of the overall paper, I think just one questions is ok since this isn't a qualitative study alone.}

We examine the discussions related to E2EE and privacy in communication apps on various Reddit forums.  We acknowledge that most users providing advice or expressing their thoughts on the privacy aspects of communication applications would be technical people that might not represent the general understanding of the masses. However, most of these discussions are initiated by non-technical people who want to understand the privacy consequences and ways to mitigate them. As these discussions train the mental model of curious non-tech people, studying these discussions could help us understand the thought process of adviser, which are eventually learned by receptive.  



% Lack of control over their privacy
% https://www.bitdefender.com/blog/hotforsecurity/facebook-leaks-data-including-private-conversations-from-50-million-accounts/

% \subsection{Analysis of Reddit discussions}

% We analyze discussion threads on Reddit across various forums that discusses E2EE, popular apps such as Slack, discord, WhatsApp, Signal, emails, Telegram, Signal and relatively unpopular apps matrix, Element, revoltchat. 





% We perform sentimental analysis for specific categories to understand people's feelings about specific topics such as E2EE. Are most comments +ve pr -ve?

\subsection{Methodology}


\subsubsection{Dataset}


We examined discussions on the privacy of online communication platforms from three prominent subreddits: "privacy" with 1.3 million members, "privacytoolsIO" with 206k members, and "privacyGuides" with 55.3k members. To filter out relevant posts for analysis, we used common keywords related to secure communication, such as "e2ee" and "messaging". We also included various communication apps with different properties, such as "Signal", "WhatsApp", "Telegram", "Discord", and "Microsoft Teams", to gain insight into users' thoughts about these apps and their properties.

We performed keyword-based filtering across these three subreddits for the last three years, resulting in 5,298 posts. We converted all posts to lowercase and made string comparisons. For phrases longer than one word, we checked if the words in the phrase occurred within a single sentence in a post. This approach minimized false negatives but generated some false positives, which we removed manually later. The mean number of comments per post was 13.86, and the mean score (the difference between upvotes and downvotes) was 43.66. However, 75\% of the posts had less than 13 comments and a ten score.
% \ks{What is score?}

We initially selected a random sample of 100 threads for manual analysis and continued adding ten new samples until we reached saturation in new codes. We aimed to consider all posts, regardless of their popularity. However, a post with multiple upvotes signifies multiple people's opinions. To take this into account, we created a pool of posts to select a random sample for analysis, with each post represented in the pool as many times as its score, which was the difference between upvotes and downvotes. Two researchers independently coded all the posts and their comments and resolved differences through discussions. We stopped coding when we reached saturation and found no new sets of posts or comments that added new codes. In total, we analyzed 210 posts with 98.5 average comments each.

% \ks{The selection method seems reasonable. For saturation, can we say exactly what post was the last one to introduce a new code?}
% \tarun{We added in groups of 10. Posts between 180-190 introduced the last codes.}
% \ks{OK. So last 5\% of posts had no new codes. I wonder if you had done a few more if something new would show up?}

% In our study, we analyze the discussions related to privacy of online communication platforms on three popular subreddits, namely "privacy" with 1.3M members, "privacytoolsIO" with 206k members, and "privacyGuides" with 55.3k members. 

% To filter a set of relevant posts for analysis, we used common keywords related to secure communication such as "e2ee", "messaging". Additionally, we included various communication apps with different properties such as, "signal", "whatsapp", "telegram", "discord", "microsoft teams" to gain insight into users' thoughts about these apps and their properties. We convert all the posts to lowercase and make string comparisons. For phrases longer than one word, we check if the words in the phrase occur within a single sentence in a post. These gives us some false positives but minimize false negatives. We can remove the false positives while analyzing them manually later. Keyword based filtering across these three subbreddits for the last 3 years gives us 5298 posts. The mean number of comments is 13.86 per post and the mean score is 43.66. However, 75\% of the posts have less than 13 comments and a ten score.

% For manual analysis, we randomly sample 100 threads initially for analysis. And keep adding 10 new samples till we reach saturation in new codes.  In our analysis, we want to consider all the opinions, even if they are not widely popular, but we also want to make sure we put equal weightage on every opinion while sampling. We created a pool of posts to select a random sample for analysis. In the pool. We put each post as many times as they their score.  The score is the difference between upvotes and downvotes. As the upvote means that those users agree with the author's opinion, analyzing one comment could help understand multiple people's perspectives. Two researchers manually independently code posts and comments and resolve differences through a round of discussions. We stopped coding when we reached saturation and found no new sets of posts or comments that added new codes.





% total posts for the last three years with any of 7 terms: 5298
% The mean number of comments is 13.86 per post and the mean score is 43.66. However, 75\% of the posts have less than 13 comments and a ten score. In our analysis, we want to consider all the opinions, even if they are not widely popular, but we also want to make sure we put equal weightage on every opinion while sampling. We created a pool of posts to select a random sample for analysis. In the pool. We put each post as many times as they their score. 

% When 10 new posts do not add new codes we stop our analysis assuming saturation is reached.



The initial phase of our analysis reveals that users strongly prefer communication apps that offer both E2EE and open-source features. In the subsequent phase of our investigation, we conduct a quantitative assessment of the user bases of popular communication apps for personal and business needs. We categorize apps based on  properties: E2EE/non-E2EE and open/closed source characteristics. Then, we find the average number of active users per app in each category and the total number of users across all apps in each category. For some apps, we did not find active users; therefore, we do not count those apps' user base while calculating average or total active users. It should be noted that these data are taken from various sources cited in the table and are calculated at different times. Our objective is not to provide exact user numbers for each app or category but rather to compare and contrast the adoption across different apps and categories as shown in Table~\ref{table_app_anaysis}.

% Furthermore, we find users' sentiments towards these apps from Reddit discussions or posts. For each app, we search the posts and comments across the whole of Reddit to calculate users' sentiments towards that app. However, one post/comment could have discussed multiple apps with different sentiments. Therefore, we use aspect-based Sentiment Analysis to determine users' sentiments toward specific apps.




    % We analyze three relevant popular subreddits: (1) "privacy" with 1.3M members, (2) "privacytoolIO" with 20k 206k members and "privacyGuides" with 55.3k members. People discuss various privacy-related topics on all these subreddits that might not directly relate to online communication platforms. To shortlist the posts for analysis, we use common keywords related to online messaging, such as "e2ee", a combination of various phrases such as a combination of words from each of the two categories "secure/private/privacy/security/" and "communication/message/messaging." Furthermore, we also include various sets of communication apps with different properties to find users' thoughts on these apps and their properties. The apps we included are "whatsapp", "signal", "discord", "slack", "microsoft teams". 




    % We search all comments and posts for these keywords to minimize the false negative. We can remove false positives while performing manual qualitative analysis. We convert all the posts and comments to lowercase and make string comparisons. For phrases longer than one word, we check if the words in the phrase occur within a single sentence in a post or a comment. Researchers manually code posts and comments and resolve differences through a round of discussions. Researchers stop coding when new set of posts/ comments do not add new codes consistently and reach saturation. 

    % From the first part of the analysis, we learn that people prefer E2EE and open sources apps most. In our analysis, we quantify users sentiments towards the apps in different categories based on the combination of these two properties E2EE/non-E2EE and open/closed source. Using various resources over the Internet, we find five popular apps in each of these categories for both personal and business uses. Furthermore, we find users' sentiments towards these apps from Reddit discussions or posts. For each app, we search the posts and comments across the whole of Reddit to calculate users' sentiments towards that app. However, one post/comment could have discussed multiple apps with different sentiments. Therefore, we use aspect-based Sentiment Analysis to determine users' sentiments toward specific apps.
    
    
    % We then get the number of user each app category has. 
    % In the second part of the analysis, we analyze 5 apps 


    
    
    Our analysis might only be a representation of more technical or motivated people who want to secure their communication and want to involve in discussions to make an informed decision.


\subsubsection{Data analysis}
We use open coding to identify the list of topics, followed by thematic analysis to identify the pros and cons of deniability. To ensure inter-rater reliability, both researchers together coded all the posts and comments and discussed and reconciled all coding discrepancies. Our goal is not to draw generalizable conclusions about the prevalence of specific issues but to identify some users' concerns regarding communication apps. 



\subsection{Qualitative results}

% \subsubsection{RQ1}


\paragraph{Conflicting opinions on the best way to achieve privacy}
We found that users' opinions on how to achieve their privacy goals often differed, even when their goals aligned. This was especially true in situations where it was not clear which app was more privacy-focused, which led to conflicts among users. For example, some users preferred Telegram over WhatsApp because Telegram is open source and, therefore more trusted. However, others preferred WhatsApp over Telegram because it provides end-to-end encryption by default and across multiple devices, whereas Telegram does not provide E2EE on desktop clients. These conflicting opinions led to fragmented user bases across different applications, out of which some were non-E2EE, making achieving widespread adoption of E2EE challenging.
\ks{What is this last point? It makes it difficult for everyone to adopt the same app? Do we already have widespread adoption of E2EE, just not everyone on the same app?}
\tarun{Some people have a different opinion of "being secure." For example, some people think telegram is more secure even if it is not E2EE because it's open source. And some users choose one E2EE over another app based on the location of their headquarters. So this causes fragmented users based across these E2EE and/or open-source apps.}
\ks{So is this last point focused on the fact that there is a mix of E2EE and non-E2EE and it is hard to get everyone using some form of E2EE? Is the message that it is hard to get most people to adopt a single E2EE app?}

\paragraph{No visible difference in E2EE and non-E2EE apps}
Although many apps claim to offer end-to-end encryption (E2EE) and are open source, users often express skepticism about the level of privacy these apps provide. This is partly due to the current user experience (UX) in these apps and the way encryption is implemented, which may not directly convey the meaning of E2EE to users. As a result, users are unable to discern what new security features these apps offer that were not available in previous apps that suffered from data leaks and breaches. Non-expert users who lack extensive experience with privacy or security technologies are especially hesitant to trust E2EE. They find it difficult to accept that some apps are more secure than others. One of the main reasons for this lack of trust is that there is often no visible difference in terms of privacy between apps that offer E2EE and those that do not.
\ks{The paragraph repeats the idea that users doubt E2EE apps. It says "users often express skepticism" this seems too strong based on small reddit sample. Some users express skepticism. Some users are skeptical? Make this point more succinct.}

\paragraph{Costs of switching to privacy-enhancing apps: Contacts, Features, and Learning}
Many users expressed a desire to use privacy-enhancing apps for sharing their data online, but the high costs associated with switching to these apps often prevented them from doing so. Three primary costs were identified: first, the cost of contacts, as all of their friends and family were using an insecure app and were not willing to switch to a different app due to convenience, preferred features, or a lack of trust in less popular apps. Second, the cost of features, as switching to a secure app meant giving up important features that were convenient or essential for business use. \ks{What is an example of these features? I don't fund that mentioned anywhere here.} Third, the learning cost, as many users, particularly non-technical individuals, found it challenging to adapt to new apps after becoming accustomed to a particular app. Users frequently voiced concerns that switching apps solely for privacy or security reasons is not practical. 


    \begin{quote}
            ``\textit{I have dumped almost all other messaging apps in favor of Signal. However, one app that I could not get away from was Viber, mainly because my close family uses it and they've grown too used to it to even discuss a change.}''
    \end{quote}


    \begin{quote}
            ``\textit{Discord is going to be like YouTube for me. I'll still use it because there's no good alternatives.}''
    \end{quote}

    \begin{quote}
        ``\textit{Literally none of my friends want to switch to matrix, I tried convincing them but they refuse, they don't care about privacy and gladly trade it for the features that discord allows. Unfortunately there is no current alternative that is better or equal to discord, otherwise people would switch.}''
    \end{quote}


\paragraph{Secure apps are censored}
The need for privacy-focused communication apps is greatest in countries with high levels of censorship. However, many of these apps are banned in these countries, which forces users to rely on less secure communication options. This creates a challenging situation where those who need secure communication the most are the least able to access it due to government restrictions.

    \begin{quote}
        ``\textit{What is the use. My country will simply ban the app.}''
    \end{quote}

\paragraph{Trying to limit secure apps to prevent fragmented user bases}
The fragmentation of users across various secure apps is a concern for privacy advisors, who fear that this could impede the widespread adoption of end-to-end encryption. This goes against the interests of non-expert users, who seek apps with specific features and may lose interest in E2EE if only recommended apps without those features. Attempting to steer everyone towards a set of apps could lead to issues such as users being dissatisfied and abandoning the apps or secure apps being acquired by entities that users do not trust, as seen with WhatsApp's acquisition by Facebook. Limiting users to specific apps could cause more harm than good. In the long term, it is important to ensure that individuals can use any app they prefer, with the features they desire, while still maintaining privacy and security in an application-independent manner.
\ks{This item is related to the second item in this section. Perhaps have them next to each other. We should study to see if they should be combined, and the points need to be clearer as to what is being said. I'm not finding these as simple and clear as the other points in this section. }
% Interestingly there might be some other apps with better features, but privacy advisors recommend the popular apps to prevent fragmented user bases across these apps. 

\begin{quote}
    
    ``\textit{if we wanna get people move to a more secure platform we shouldn't get too fragmented. Otherwise we'll end up with having so many apps just because this one friend likes app A and the other one likes app B. It could make people less likely to move away from WhatsApp because there's just so much choice.}''

\end{quote}

\ks{I don't understand the last sentence from this user. We can't edit it, but how does it help the point we are trying to make?}
\tarun{The last sentence says that privacy experts who advise others have  different preferences for secure apps. Because there are so many secure options, people advise different apps. Non-experts get multiple suggestions for applications; for example - a user A who uses WhatsApp is suggested by friend B to use signal and suggested by friend B to use Telegram. User A gets confused and chooses not to switch to any app and continues to use WhatsApp.}


% \subsubsection{RQ2}

    \paragraph{Closed sources}
        % Even if an app claims to be secure and implements E2EE, users do not implicitly trust them more than other apps if it is a closed source. As users cannot verify app's claim regarding privacy and security, no use of trusting these apps more than others. This is a real issue, because there are many apps which have proprietary code which prevents thaem from open sourcing their code. 
        
        % There are a few valid reasons for many apps not to release the source code of their apps. One of the major to protect their Intellectual property. The apps may contain proprietary code that provides a competitive advantage to the app creator. Open-sourcing code could result in the loss of this advantage and make it easier for competitors to copy or imitate their app's functionality. Open-sourcing the code could make it difficult to enforce intellectual property rights and could result in legal disputes. 

        % There needs to be work done to isolate the encryption code from the other proprietary code nad make it open source. This will increase users trust in these apps implementing E2EE. 

        Closed-source apps claiming to be secure and implementing E2EE do not automatically garner users' trust. Since users cannot verify the app's privacy and security claims, trusting these apps more than others is futile. However, many apps cannot release their source code due to proprietary code that offers a competitive edge to the creator. Open-sourcing the code could lead to loss of that advantage and legal disputes. Therefore, there is a need to segregate the encryption code from other proprietary code and make it open source. This approach would help increase users' trust in apps that implement E2EE.

        Even if an app such as Telegram does not implement E2EE by default is trusted more than WhatsApp because its open source.  

\begin{quote}
    ``\textit{Telegram is better than Whatsapp. Atleast it’s open source.}''
\end{quote}


    \paragraph{Lack of trust in E2EE client's app}
    Users have expressed concerns about the client end of apps implementing end-to-end encryption (E2EE) having access to their plaintext data. This concern appears to be more prevalent in closed-source apps, but also exists in open-source apps. Users were apprehensive about the possibility of the client end processing their data by loading dynamic codes, even if the app's source code is open for review. Such concerns indicate the need for greater transparency in the way these apps process user data, including the ability for users to monitor the data processing activities at the client end.
    
    

    % \paragraph{Lack of trust in E2EE due to client's app control on encryption}
    
    %      If an app claims to implement E2EE, users do not implicitly trust them more than other apps. 
    %         There are other metrics they consider more while selecting apps: 
    %             open source
    %             apps company
        
        
    %     Even apps that provide E2EE users doubt them.
    %         issue is users do not trust that app are implementing E2EE correctly and all apps might not be able to open source their client code.
    
    \paragraph{Lack of trust in algorithms an app use}
        Users have expressed concerns about the use of encryption algorithms by certain applications, particularly Telegram. This is due to Telegram's proprietary encryption algorithm being broken in the past by security researchers, leading users to question its reliability and trustworthiness even after updates. Users have expressed a preference for alternative encryption algorithms that they consider to be more secure. Additionally, users desire greater flexibility in selecting different encryption algorithms for the apps they use, which can help increase the adoption of secure apps and improve user satisfaction. These findings highlight the importance of providing users with a range of encryption options that they can choose from to enhance their trust in the security of the apps they use.

    \paragraph{Incomplete}
        A lot of users are interested in securing or making their data more private for various applications. Currently, they need to find and use different apps that provide E2EE for each use case such as writing notes, and contact syncs. Furthermore, some encryption platforms do not provide the completeness that users prefer such as proton mail does not encrypts Subjects in emails. Finding different apps and verifying them for different uses is very cumbersome for users. 

        \begin{quote}
            ``\textit{Am I crazy to be worried about my privacy when it comes to note taking apps?}''
        \end{quote}

% \subsubsection{RQ3}

\paragraph{Users' trust biased based on owners' reputation}
When two apps have similar properties, such as both claiming to implement end-to-end encryption (E2EE) but neither being open source, users are more likely to distrust the app owned by someone with a bad reputation. The reputation of the app's owners is an important factor that users consider when assessing the trustworthiness of apps with similar features.
\ks{Last two sentences have some redundancy. Maybe we can improve.}

\textit{
    ''\textit{The privacy issue with Whatsapp is, it's owner by Facebook which is exactly opposite of privacy and now whatsapp will share the data with it.}''
}

\paragraph{Elimination method}
there are tons of alternatives available for communication in the market, and none of them are absolutely secure. Therefore, most users tend to choose apps using elimination methods by discarding a set of apps they do not want to use based on certain factors. The most common factors considered while eliminating apps are (1) open source or closed source, (2) E2EE by default (3) the owner's reputation, (4) the app's historical reputation, and (5) the location of the app's company. Users dynamically reevaluate these factors whenever something changes for example when WhatsApp was bought by Facebook, they started trusting WhatsApp less and when Telegram moved their headquarters to Dubai users doubt their intentions. 


\begin{quote}
    ``\textit{Telegram is evil, not automatically E2E and based in dubai middle eastern governments will savagely hack those servers some day}''
\end{quote}


\begin{quote}
    ``\textit{Rakuten (the owners) do collect metadata. But then again, they are not Facebook and are not American, so that alone makes them a lot more trustable than WhatsApp/FB Messenger.}''
\end{quote}



\section{Communication platforms analysis}
% We analyze the status of status of popular communication platforms in personal and business use. The two most important factors that determines an application's privacy are if an app is E2EE and open source. We categorize 23 popular personal apps and 25 popular business apps into combination of E2EE and open source category. Apps with both personal uses are categorized separately. 
% Table~\ref{table_app_anaysis} shows that none of the app among the list of these popular apps is E2EE and open source. Among personal apps, only three implement E2EE by default. Five apps have optional E2EE and one app- Telegram is open source among them. 15 personal use apps do not provide E2EE and are closed source too.

% For business uses cases we found even worse E2EE adoption. Only two apps implement E2EE by default and one app provides it as an option. The lack of adoption of E2EE is concerning as many companies who uses these communication platforms shares/exchanges users sensitive data. Using E2EE for business communication is as important as personal communication if not more. Currently, users give access to their data to specific apps/companies. If these companies use other communication platforms internally or with customers to exchange these data, these third party companies would have access to users sensitive data that they they never wanted to share to these third party companies. 

% \ks{Should the reddit study appear before this section as motivation for why we looked at E2EE and whether it was open source? Otherwise, why do we focus on these two properties? "We identified two properties" how and why?}


% We conducted an analysis of reddit threads to gather user requirements and preferences for an E2EE system. This revealed certain properties. Then the analysis of the apps is partly motivated by what we learned, that users desire and trust open source implementations.

From our analysis of Reddit threads, we learned that because there is no visible encryption on the current application, users rely on the following two key properties to determine the privacy of an app: (1) E2EE and (2) open source. A user trust most an app that is E2EE and open source and they trust least an app that is not E2EE and not open source. 

In this analysis, we analyze popular applications both in personal and business domains based on the above two metrics to identify if users believe transfer to real usage of their applications or not. We try to identify if even after knowing which app is more secure, they cannot switch to those applications because of reasons identify in the Reddit analysis study. 

% provided us with two criticial properties that users use 

% In our study, we analyzed the privacy status \ks{Will think about whether another term is more appropriate than status. Are we rating the privacy of these applications based on whether they offer these two properties? Is it privacy and trust? Open source means there is potential for independent security analysis. Is that the big reason it is important?} \tarun{Yes! Open source allows to confirm that they really provide E2EE by verification of their source code.} of popular communication platforms widely used for personal and business purposes. We identified two key factors that determine the privacy level of these applications: whether the app is end-to-end encrypted (E2EE) and whether it is open source. 
% \ks{E2EE makes sense. Need an explanation of how open source is a property relevant to privacy status.}

We categorized a total of 23 personal apps and 25 business apps based on their combination of E2EE and open-source status. We further categorized the personal apps separately from the business apps and a third category of apps used for personal and business use.

Our findings, as shown in Table~\ref{table_app_anaysis}, indicate that none of the popular communication apps we analyzed are both E2EE and open source. Among the personal apps, only three implement E2EE by default, while five apps offer E2EE as an optional feature. Telegram is the only app among these that is open source. The remaining 15 personal apps do not provide E2EE and are also closed source. 

For business use cases, we found even worse adoption of E2EE. Only two apps implement E2EE by default, and one app provides it as an option. The lack of adoption of E2EE is concerning, as many companies rely on these communication platforms to share and exchange sensitive data. The use of E2EE for business communication is just as important as it is for personal communication, if not more so. Currently, users grant access to their data to specific apps or companies. \ks{What does it mean to grant access to a company? Is this when I use one of these tools to communicate with customer service reps, like online help?} \tarun{Yes! Thats one example. Another example could be you share your health or financial records with app X, and that app uses Slack for internal communication. Depending on what kind of data is shared between employees of app X using Slack, users' data could be at risk.} If these companies use other communication platforms internally or with customers to exchange this data, third-party companies may gain access to users' sensitive data, which users never intended to share with those companies.

All the applications we analyzed, including the ones that are E2EE, assume trust in their client application. This is an issue in the long term because why trust clients if we don't trust servers?



\input{table_apps_analysis}


==> analysis.tex <==
\section{Analysis}


10-20 users suffice for usability testing to detect atleast 80-95\% usability issues.
https://link.springer.com/content/pdf/10.3758/BF03195514.pdf

==> comparison_table_old.tex <==
\newcommand*\rot{\rotatebox{90}}

% \newcolumntype{R}[2]{
%     >{\adjustbox{angle=#1,lap=\width-(#2)}\bgroup}
%     l
%     <{\egroup}
% }
% \newcommand*\rot{\multicolumn{1}{R{90}{1em}}}


% \newcommand*{\yes}{{\tiny \CIRCLE}}
% \newcommand*{\no}{{\tiny \Circle}}
% \newcommand{\sometimes}{{\tiny \LEFTcircle}}

\begin{table*}[h!]
\caption{\sysname comparison with existing E2EE systems.}
\begin{center}
\label{table:system_comparison}

\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|c| c c c c c c| c c|c c c c|}
\hline
&\multicolumn{6}{c|}{Security} & \multicolumn{2}{c|}{Scalability} & \multicolumn{4}{c|}{UX}  \\
\hline
% \cmidrule{3-6}%
E2EE systems & \rot{Prevents server access} & \rot{Prevents passive client attacks} & \rot{Prevents active client attacks} & \rot{User controls encryption} & \rot{Easy security evaluation and patching} &
\rot{Application independent} & \rot{Requires no per-app configuration} & \rot{Supports developer API} & 
\rot{Supports selective encryption} & \rot{Supports visible encryption indicator} & \rot{Supports visible isolated encryption}  & \rot{Preserves target application UX}
\\

%  E2EE systems & No plaintext access to client app  & No app support required & Scalable & Encryption support for developers & Original app's UI experience & forward secrecy & Ease of patches\\
\hline

PGP, S/MIME & \yes & \no  & \no  & \no & \sometimes & \no & 
    \yes & \no & 
    \no & \no & \no & \yes\\
% S/MIME & \sometimes & \no  & \no & \no & \sometimes & \no & 
    % \no & \no & \no & \yes&  % users requires certificates from CA
    % \no & \sometimes & \no \\
OTR, Signal, WhatsApp, TextSecure, Gibberbot  &  \yes & \no  & \no  & \no & \sometimes & \no & 
    \yes & \no & 
    \no & \no & \no & \yes\\
FlyByNight & \sometimes & \no  & \no & \sometimes & \sometimes & \no & 
     \yes & \no & 
    \no &\no & \no & \yes\\
% GOTR\\


% Babelcrypt & \yes & \sometimes & \yes & \no & \yes & \yes & \no & \no & \no & \yes & \sometimes & \yes & \sometimes\\

\textdagger Shadowcrypt, 
MessageGuard, 
Virtru & \yes & \yes & \no  & \yes & \yes & \yes & \no & \no & \sometimes & \yes & \no & \sometimes\\
% Fahl et al.~\cite{fahl2012confidentiality}\\

\textdaggerdbl Mimesis Aegis, Babelcrypt & \yes & \yes & \no & \yes & \yes & \yes & \no & \no &  \sometimes  & \yes & \no & \sometimes\\


\sysname & \yes & \yes & \yes  & \yes & \yes & \yes & \yes & \yes  & \yes  & \yes & \yes &\no\\

% WhatsApp potentially accepted as evidence &&&&&\\
% \hspace{3mm}Civil cases&&&&&\\
% \hspace{3mm}Criminal cases&&&&&\\

% \hline
% WhatsApp potentially rejected as evidence&&&&&\\
% \hspace{3mm}Civil cases&&&&&\\
% \hspace{3mm}Criminal cases&&&&&\\

\hline
% \multicolumn{4}{l}{${*}$ login session is very short lived}\\
\end{tabular}
}
\end{center}
 % \vspace{1mm}
\hspace{10mm} \textdagger~= Only works for websites in Browser.

\hspace{10mm} \textdaggerdbl~=Only for phones. Cannot be adapted to PCs directly. Included in the comparison for completeness. 
\tarun{I propose combing PGP and OTR rows, and Shadocrypt and Mimesis rows. they both have same properties. We can only have these two rows (1) E2EE protocols and (2) Browser \& Phone based E2EE systems. We can also consider removing FlyByNight.}
% \ks{Use consistent capitalization and improve names for all the column names. Are all the others only for desktops like InfoGuard, or do some work on both?}


% \vspace{1mm}

\end{table*}

==> design_old.tex <==
% \section{System design}
% Our idea is to provide support for OS-to-OS encryption to all applications in a scalable manner - scalable to all inputs and applications. When a user inputs into an application through any input devices like a keyboard, Hard drive, the OS encrypts the data before it reaches the application. The application sees only encrypted data and forwards it to the intended recipient over the internet. The recipient's application also sees the encrypted content, however before it reaches the display or to any output device, the content is decrypted. 


% \tarun{Threat Model: our goal is to protect sensitive data from benign clients' app. Honest but curious adversary.}

% \paragraph{\bf Our goals:} 
% \begin{enumerate}
%         \item Enable developers to enable E2EE to any input field for their application written in any language. 
%         \item Enable users to start E2EE on any input field of any application, assuming the application to be malicious. 
%         \item Support direct administrator control over the parameters and settings for E2EE connections made by our system. Applications should be able to increase, but not decrease, the security preferred by the administrator.
%         \item complete data and logic isolation from untrusted entities; Current E2EE like signal trust the client apps of untrusted entities. If we do not trust server, we should try to stop client apps too. 
%         \item Applicable to all communication apps like email, messaging apps, Slack, Microsoft team chat, zoom chat, Netflix watch party chat, etc. Previous research~\cite{abu2017obstacles} shows that usability is not the primary obstacle to adoption, fragmented users bases and lack of interoperability are significant obstacles.
%         \item Preservation of original user experience with target apps, but involve users in encryption and decryption process. Previous research~\cite{ruoti2013confused} shows that reducing transparency by requiring manual encryption from users led to fewer mistakes and an increase of trust in the security of the system.
%         \item Developer Malfeasance: The developer of a communication application could transmit user data to a third-party without user consent. The proposed system allows users to encrypt their communication with end-to-end encryption and see the encryption process happening in real-time, increasing user trust and reducing the likelihood of developer malfeasance.
% \end{enumerate}





% \subsection{User interface design goals}
% \begin{enumerate}
%     \item Users reject security protocols or advice if they perceive the additional effort is not worth the extra security they get~\cite{herley2009so}. 
%     \item Users lack the knowledge to obtain, distribute, or use cryptographic keys~\cite{whitten1999johnny, sheng2006johnny}.
%     \item Users trust manual encryption more than transparent encryption; they do not know if/how the system works.~\cite{ruoti2013confused} shows evidence that manual encryption can foster greater trust and reduce user errors.
%     \item Users believe that desktop applications are less likely to transmit their personal messages back to the developer of the software~\cite{atwater2015leading}.
%     \item Research has shown that most users are not interested in encrypting all of their online data~\cite{gaw2006secrecy, ruoti2013confused}. As such, users must be able to control when their data is encrypted.
% \end{enumerate}
% As described in usability consideration section, users trust manual encryption more than transparent encryption. We observed the following critical differences in the manual encryption as compared to the transparent encryption: OB1: User's can see the encrypted text which ensures that encryption is performed, and OB2:) Users pass only encrypted text in the application's text box, which ensures them that the application never sees their plain text data.

% Based on point 1 from user interface design section, user also rejects security protocols if they perceive the additional effort is not worth the security. So, to maximize the chances of acceptance of our system, we have to minimize the effort while providing OB1 and OB2. 

% In our system, we plan not to make any GUI changes to the applications, allowing users to get the same UI experience as without encryption. We plan to use a keyboard shortcut to provide a consistent UX for encryption and decryption across all applications. We are also providing selective encryption to every textfield; a user can press the encryption shortcut to start or stop encryption at any point while typing. After a user initiates encryption, our system shows encrypted text in the application and plaintext in our system's isolated GUI. Isolating our GUI from browsers and other applications would convey the fact to the users that the encryption is isolated from the application and browsers. 
% Also, the user should be able to notice that the application never had access to plaintext. 


\subsection{System design}


% \subsection{Challenges}
% \paragraph{Data decryption on the receiver end}: 
% Ideally, we would want to decrypt the data at the kernel layer just before it is being displayed on the screen. However, currently, the GUI rendering is handled in the user space at the library used by X client. If we decrypt the data just as soon as it leaves the application by hooking code in Xlib, there are two issues: (1) the X server would have plaintext data that could be accessed by all other user-space applications, (2) the decryption process will be transparent to the user which violates our one of the design goal.

\paragraph{Encryption algorithm selection}
Currently, Signal protocol uses AES CBC for encryption, which is block cipher. For our system, we require a stream cipher because to achieve OB1 and OB2, one-to-one mapping of a plain and cipher character would convey the existence of encryption to the user. 

We decided to transition to adapt AES-OFB, a stream cipher, into Signal. 

Our current implementation doesn't require a stream cipher at all, only a one-time pad with which to XOR. When a new plaintext comes in to the system, the program first checks if the one-time pad is long enough. If it is, it XORs the one-time pad with the plaintext to create the ciphertext. If it isn't, the system creates more of the one-time pad by encrypting a sequence of 0's. This elongated one-time pad is then XORed with the plaintext to create the ciphertext.
In other words, as long as there is some kind of mechanism to deterministically create the next portion of the one-time pad, it really doesn't matter whether the cipher is a block or stream cipher. Ideally, of course, I would submit the updated plaintext to the stream cipher directly and get the updated ciphertext, but the OpenSSL implementation assumes (correctly, I might add) that most people don't want to edit the earlier parts of the plaintext. I could potentially repeatedly create and destroy the OpenSSL cipher to get a fresh start, but that feels less than ideal to me.
I have this fuzzy memory that using an XOR pad is a bad idea. Are there issues with using an XOR pad? Should I find a solution that uses only OpenSSL, even if that means repeatedly creating and destroying the cipher? I guess I could look for something that clears out the intermediate ciphertext, but I doubt that exists.


\paragraph{Handling encrypted text editing}
\tarun{Discuss w/ Justin}

\tarun{Following code updates 5th character. Is it wrong? ALso, instead of 0, need to use IV. Does signal protocol already shares IV?}

unsigned char key[16] = "0123456789abcdef";
    unsigned char iv[16] = "fedcba9876543210";

    // Encrypt the plaintext "hello world"
    unsigned char plaintext[11] = "hello world";
    unsigned char ciphertext[11];
    int ciphertext_len;
    EVP_CIPHER_CTX *ctx = EVP_CIPHER_CTX_new();
    EVP_EncryptInit_ex(ctx, EVP_aes_128_ofb(), NULL, key, iv);
    EVP_EncryptUpdate(ctx, ciphertext, &ciphertext_len, plaintext, sizeof(plaintext) - 1);

    // Update the 5th character to "z"
    plaintext[4] = 'z';
    EVP_EncryptUpdate(ctx, &ciphertext[4], &ciphertext_len, &plaintext[4], 1);"

Most encryption systems assume that any prior encrypted data does not need to be edited. Since OSI supports editing the plaintext anywhere, the system has to use a slightly modified encryption scheme.

The C implementation of Signal OpenSSL's implementation of AES-CBC for encryption. During initial development, we knew that we would need more flexibility. The original vision was to have a system where it was clear that every single character corresponded to a single character update, and a stream cipher fit the bill exactly. After realizing that Signal already MACs the message, we decided to go for AES-OFB.

However, we did not anticipate how unorthodox it is to edit portions of the plaintext that have already been encrypted. OpenSSL's EVP\_EncryptUpdate() assumes that the next portion of data to encrypt starts at the next byte in the overall plaintext. To get around this issue, we caused the system to generate a one-time pad which is then XORed with the plaintext to create the ciphertext. When a new plaintext enters the system, the program first checks if the one-time pad is long enough. If the one-time pad is long enough, the program XORs the one-time pad with the plaintext to create the ciphertext. If the one-time pad is not long enough, the program encrypts a long enough sequence of zeros as the next portion of the one-time pad and then XORs the one-time pad with the plaintext to create the ciphertext.

Since we must be able to edit prior portions of the ciphertext, and given this solution, it actually became unnecessary to use a stream cipher. Whether using a stream or a block cipher, what is actually needed is a way to deterministically obtain a one-time pad on both sides, and either a stream or a block cipher fulfills that requirement.

The other way around this issue would be to somehow reset the OpenSSL context encryption location but not the key or IV before each encrypt. I'm not sure yet if this is possible, but it would be ideal. It would also be relatively straightforward to repeatedly create and destroy the entire OpenSSL encryption context while encrypting, but then all of the prior encryption work would have to be performed again. By using the one-time pad, the system has to encrypt up to only a few more bytes as there are in the plaintext.

% \subsection{Language support for applications}
% Our system is based on trigger mechanism, unlike secure socket API. Therefore, supports all languages by default. 

% \subsection{Searching encrypted data}


 
 
%  \subsection{Why user involvement in encryption?}
 
 
%  three-quarters of respondents believing that their E2E encrypted communications could be accessed by unauthorized entities.
%  https://www.usenix.org/conference/foci18/presentation/abu-salma. Can we change this mental model by showing encrypted text in app and plaintext in separate window. 
 
%   users hold a belief that desktop
% applications are less likely to transmit their personal messages back to the developer of the software.https://www.usenix.org/system/files/conference/soups2015/soups15-paper-atwater.pdf

% So, by (1) giving users the control of encryption users and (2) encryption handle by the system, could increase trust in the encryption system. 

==> implementation_old.tex <==
\section{Implementation and Performance}

% Talk about what we did for proxy implementation

% \ks{One quest I have is does the proxy mechanism work with a variety of applications (the app doesn't obscure the content such that the keyword replacement approach breaks, for instance). Are there other measurements we can think of? Maybe make a list, which could be for the future.}
% \tarun{According to my understanding, applications do not obscure the data they send from their app to their server. They might use different variants of protocols for communication, such as HTTP2, HTTP3, sockets, QUIC. We just need to write down intercepting code for all these popular protocols. MITMproxy allows us to do that. Some apps might use different encodings to make it easy to transfer data, but these are relatively easier to account for. In future we can do measurements across 40-50 apps and see how many we can successfully intercept. Maybe we find something that we don't expect.}
% \tarun{We have successfully tested our MitM proxy with different websites such as discord, slack gmail. It also works for outlook client app.}



We build a laboratory-based prototype implementation of \sysname to demonstrate its feasibility, evaluate its performance and effectiveness. Our implementation of the Interceptor is a native C/C++ application that runs the GUI and the MitM proxy as a child process. We employed the Tkinter Python library for Tcl/Tk to develop a user-friendly and adaptable design with cross-platform compatibility for the Interceptor GUI. We utilized the Signal's C library (libsignal-protocol-c)~\cite{signalclibrary} to implement forward secrecy encryption and decryption, which we modified to perform stream cipher. 
% \ks{The term conducted at the beginning seems inaccurate. We conduct users studies, but here we develop or implement a prototype. Do we want to claim it is user-friendly since we provide no user study?}



\subsection{\sysname message flows}

% \ks{This section jumps to low-level implementation details. I prefer a systems paper with a clear separation from design and implementation. Not sure it is possible with something at the system level like this is.}

\paragraph{\sysname's initialization}
In Unix-like operating systems, the \textit{/dev/input} directory contains device files for input devices such as keyboards and mice. The \textit{/dev/input/eventX} files are event files that correspond to input devices, with X being a number that identifies the specific device. A keyboard input file allows applications to receive raw keyboard events, including key presses and releases, without any processing or interpretation by the system. Generally, windowing systems such as Window System (X11) API or the Wayland protocol in Linux read keyboard input files, and applications receive keyboard input events from the windowing system.

To intercept the keyboard input, our system opens the relevant keyboard event file (e.g., \textit{/dev/input/eventX}) in a read-only, nonblocking mode. Then, it creates a virtual keyboard using \textit{uinput}, which it later uses to pass encrypted messages to the target application. The \textit{uinput} interface in Linux allows programs to create virtual input devices and send events to them through the /dev/uinput device file using the uinput API. Once created, events are sent to the virtual keyboard using the write system call, and the kernel receives them as if they were coming from a physical keyboard. 
% Finally, using \textit{Xlib} functionality, the interceptor creates a new X window of no dimension. \tarun{Why?}

% Using the file descriptor, the program creates two Libevdev structs: one representing the actual physical keyboard (struct libevdev kbd\_phys) and one representing the virtual keyboard (struct libevdev\_uinput kbd\_virt) through which the program will later send the encrypted message. The interceptor creates a new X window of no dimension using Xlib functionality.
% The interceptor creates a new X window of no dimension using Xlib functionality.


\paragraph{Waiting for user to enable encryption or decryption mode}
The interceptor daemon is in place and actively listening to the keyboard input file. To detect encryption and decryption shortcuts, Interceptor employs \textit{xkbcommon}, an open-source library designed for key event processing and keymap compilation in the X Window System protocol. Interceptor compiles a keymap using xkbcommon's keymap compiler and utilizes the resulting keymap to process key events. This entails setting up an event loop to obtain keyboard events and checking the keymap's state to identify whether the encryption or decryption shortcut has been pressed. When the daemon detects the correct sequence of keystrokes, the program switches to the appropriate mode, encryption or decryption.

% \ks{Figure 3 comments. This abstraction should be the first things explained in the paper perhaps before the GUI explanations. If we removed details of the three alternatives, is there a single abstraction that applies to all in the purple part? Why the different style for lines? I don't understand arrow from first purple box to the blue box after decryption. Should there be a line from enable encryption blue box to the first purple box? What about looking for the disable encryption shortcut?}

% \begin{figure*}[t!]
% 	\centering
% 	\includegraphics[width=1\textwidth]{images/E2EE_architecture-Mitm_flow_diag.drawio.png}
% 	\caption{\sysname flow diagram.}
% 	\label{fig:seid_design}
% \end{figure*}


\paragraph{Encryption mode initialization}
We use a state-of-the-art Signal E2EE protocol that provides forward secrecy and deniability. However, \sysname cannot use Signal protocol directly because Signal uses AES-OFB block cipher and expects the entire text to be typed before the encryption process starts. Interceptor expects to display the encrypted text in real-time as the user type, indicating to users that the input is being encrypted for the app they intend to use. The AES-OFB mode can be used as a synchronous stream cipher as it generates keystream blocks, which can be XORed character by character. However, OpenSSL does not provide an API to retrieve the keystream block instead it takes a 128-bit input and returns the encrypted text (plaintext\_block XORed keystream\_block). In our implementation to retrieve the keystream, we pass a block of 0s as input to OpenSSL for encryption and XOR the output with 0s again, which is equal to the keystream that OpenSSL used internally as XOR is a reversible function. Interceptor uses this 128-bit keystream to perform character-by-character encryption by XORing it with user input. When only 16 unused bits are left in the keystream, Interceptor encrypts an additional block of 0s (128 bits) and continues this till the user finish typing in the encryption mode. The C Signal library (\textit{libsignal-protocol-c}) is used for this implementation since the overall \sysname relies heavily on system library calls, particularly related to Libevdev.


\ks{This four blocks discussion seems really ad hoc and imprecise. How long is a block? Do we mean AES block? What if user is typing something more than eight blocks? This OTP description also seems like home-grown crypto. CCS readers are going to want security proof it is correct won't they? Is this effectively an AES stream cipher mode - can we use that and describe as such? Is integrity provided already from something in Signal or is that an issue?}
\tarun{Updated.}

 Interceptor uses the Libevdev library to grab exclusive access to the keyboard input file. It gains exclusive access to the keyboard, preventing other applications or processes from accessing it until the grab is released. It is achieved using the \textit{LIBEVDEV\_GRAB} flag in Linux.
Interceptor determines the appropriate location to place the final message \ie, the application's input textbox through which the user initiates encryption mode. It utilizes XGetInputFocus() from the Xlib library to keep track of the previous input application. 
Interceptor starts the Encryptor module used for encryption and decryption. Interceptor starts the GUI module. The GUI module prompts the participants to either choose a recipient from available options or add a new recipient to encrypt their messages. 


% For \le and \de, the GUI is an interface where user sees the plain text they type. Users do not type on this interface, but target application's interface as usual. 

Once the recipient is selected, the user can begin typing in the application they wish to encrypt their message into, and the GUI displays the plaintext in real time. 

% In \os version, the GUI appears as a visible overlay on top of the entire screen when the encryption mode is enabled. The user enters the plain text they want to send through the target application on this overlay.


\paragraph{Encrypting the message}
As the user types the plaintext message, Interceptor forwards the ASCII characters to the GUI, which dynamically displays the plain text characters that users type in the target application. Interceptor maintains a list of whitelist keys, such as arrow keys or shortcuts \textit{Ctrl+A}, and \textit{Ctrl+C}, that it does not encrypt. These whitelisted keystrokes are passed to apps through the windowing system in plaintext.
\ks{I don't understand this last sentence. Why passed to the apps? I thought they just trigger the encryption process, so what is app going to do with them?}
\tarun{These are not encryption enable/disable shortcuts. These shortcuts are used for other purposes such as selecting all text, copying, pasting, etc. The whitelist keyword also includes caps lock, arrow keys, etc. }

% Interceptor encrypts the user input character by character using the modified Signal protocol to allow for a stream cipher. 
% Interceptor encodes the encrypted text and metadata with base64 to ensure that all characters are printable in the target application's textbox. Interceptor writes the base64 encoded encrypted text and metadata to the app using the virtual keyboard it created during initialization. To write the encrypted text, it first removes metadata by simulating backspace keys using the virtual keyboard and then simulates the new encrypted characters and updated metadata keypresses. We determine that the minimum gap between two consecutive virtual keypresses is 0.00125 seconds before it corrupts the kernel's internal \textit{/dev/input} ring buffer, used to read virtual keyboard inputs by the application, leading to lost keystrokes. For efficiency, Interceptor waits for 0.3 seconds after the latest user's key presses before it starts encryption. It allows more efficiency and usability by waiting for the user to finish the block of words or sentences and avoiding frequent backspacing and retyping of metadata. \tarun{What things are updated?} \tarun{What's the total length of updates?}
% \tarun{ciphertext length	ciphertext string}

% In \ds, Interceptor generates a random ASCII character for every character a user types. Interceptor passes those random characters to the target application's textbox using the virtual keyboard, as described for the \ls version. Here, Interceptor does not wait between the user's key presses as it can generate random characters efficiently at a faster rate than user types, and also, there is no metadata involved, so no deleting and retyping are required using the virtual keyboard. Interceptor keeps track of the random characters it sends to the application as a unique identifier. Interceptor dynamically synchronizes this unique identifier with the MITM proxy. The MITM proxy searches all the outgoing data from the target application for the unique identifier.


Interceptor encrypts the user input character by character using the modified Signal protocol to allow for a stream cipher. 
To ensure all characters are printable in the target application's textbox, the Interceptor encodes the encrypted text with base64. Then, it wraps the base64 cipher text in a token format: "IGS{<cipher text>}IGE". This token serves two purposes: first, it helps the MITM proxy to identify the cipher text and append metadata uniquely; second, it provides the recipient with an easy way to understand that the text is encrypted. Interceptor writes the base64 encoded encrypted text to the app using the virtual keyboard created during initialization. We determine that the minimum gap between two consecutive virtual keypresses is 0.00125 seconds before it corrupts the kernel's internal \textit{/dev/input} ring buffer, used to read virtual keyboard inputs by the application, leading to lost keystrokes. For efficiency, Interceptor waits for 0.3 seconds after the latest user's key presses before it starts encryption. It allows more efficiency and usability by waiting for the user to finish the block of words or sentences and encrypting them at once.


\sysname also needs to send metadata, such as the message length, MAC and Diffie-Hellman ratcheting keys, to the recipient along with every message. The total length of metadata is greater than 50 bytes \ie $50 + plaintextLength + floor(plaintextLength / 128) + 2*floor(messageNumber / 128)$. Adding this long metadata can negatively affect users' experience. Therefore, to append this metadata to the user's encrypted message Interceptor sets up a local MITM proxy. 

% This proxy starts scanning the outgoing messages from the app as soon as the user initiates encryption mode. Interceptor dynamically synchronizes the encrypted text with the MITM proxy. The MITM proxy searches all the outgoing data from the target application for the encrypted text and appends metadata to it before letting it pass through over the Internet.

Mitm proxy continuously listens during the encryption mode to append the metadata to the encrypted text. After the encryption mode is activated, Interceptor uses GDBus to call a custom Gnome shell addon called Window List, which retrieves a list of all open windows in JSON format. It then select the window in focus, retrieve the PID, and add it to the E2EE cgroup under \textit{net\_cls}. It then redirect traffic with destination ports 80 and 443 from this cgroup using \textit{iptables} and \textit{ip6tables} rules to port 8080, the default listening port for MITMProxy. It starts the MITMProxy process from the "mitmproxyuser" account to find the encrypted text string and replace it with encrypted text||metadata. When the user deactivates the encryption mode, Interceptor terminates the MITMProxy process, reset the IP tables, and moves the process out of the E2EE cgroup.

% In \os, the user types the plaintext message on the overlay. After the user finishes writing the message, Interceptor encrypts the message using the signal protocol. Then, it passes the base64 encoded encrypted text and metadata to the target application's text using the virtual keyboard. 


\paragraph{Encryption termination}
When Interceptor detects the shortcut to disable encryption mode, it waits for the encryption function to finish and updates the latest encrypted text and metadata in the target application's textbox. Then, Interceptor adds the ciphertext hash and plaintext mapping to the local cache. This local storage allows the user to again see the plaintext messages through the ciphertext message later. Without this, the sender will not be able to see a message after sending it, and the recipient will not be able to see it after the first decryption. To achieve forward secrecy, Signal deletes the previous keys. Interceptor cleans up the Signal encryption context. In particular, the Signal keys are appropriately ratcheted, the one-time pad is zeroed out and freed, and the underlying cryptographic structures are freed. Interceptor releases its exclusive grab of the keyboard input file, thus allowing other applications to resume reading from it. Interceptor kills the GUI.
\ks{This local cache seems like a big deal. Who has access to it, and how do users come back to these messages? What about the issue of reading messages from multiple devices? If I cache it on my phone, what happens when I read the message on my laptop?}
\ks{I think key management is a big issue that needs to be introduced earlier. I see hints about it, selecting recipients, local storage, but it isn't a primary issue in the design discussion.}
\tarun{I'll extend the key management paragraph to describe, key distribution and multi-device support.}


Interceptor waits for the MITM proxy to replace the random character unique identifier with the encrypted text if it has not been done already. Then, Interceptor closes the MITM proxy. 

% \tarun{Can we identify when a user sends messages from an application? How to prevent a user typing a message, sending and continue typing more in second message?}


\paragraph{Decryption on the receiver end} 
In \sysname, we incorporate user involvement in the decryption process to achieve translucency, which helps to increase trust in our system. As highlighted in Section~\ref{}, Interceptor actively listens for the encryption/decryption shortcut, which the user can trigger to view the decrypted message. When users receive an encrypted text, they only see the ciphertext in the application. To decrypt the message, the user selects the encrypted text and presses the decryption shortcut, which is \textit{Ctrl+Shft+U}.

Interceptor retrieves the selected text from the application using Xlib, which enables any application to retrieve selected text using the PRIMARY selection. Once the selected ciphertext is obtained, Interceptor pops up a graphical user interface (GUI) window for the user to choose the message's sender. It then uses the key session with the selected sender to decrypt the received encrypted message. Similar to the encryption mode, Interceptor pops up another GUI window to show the plain text to the users.

To ensure that plaintext is not accessible to other applications through the display server or due to vulnerabilities in the display server software itself, the GUI process directly writes the plaintext to the framebuffer. This prevents any other application from accessing the plaintext, even if they have access to the display server.

\paragraph{Developer's API}
Interceptor exposes a socket to all applications that allow them to trigger encryption. Application developers can notify the Secure Encryption ID (\sysname) through a socket to initiate encryption. To detect when a user starts typing in a textbox that needs to be secured, developers can use listener functions such as "onfocus" in JavaScript and "textbox.bind" in Tkinter (for Python).

It should be noted that the scope of this design does not include protection against attacks on the client app itself that may disable the \sysname call. However, it is important to highlight that such attacks are possible due to vulnerabilities in the application, not the \sysname system. \sysname ensures that if a user wants to start encryption, the application cannot access plaintext data even if it is actively trying. However, if the user explicitly chooses not to use \sysname, the responsibility for encryption falls on the application developer. In such cases, the level of security provided by the application's encryption mechanism is as secure as the client end of the application. \sysname runs with sudo privilege and therefore other non-sudo apps cannot delete or impersonate the socket API to perform denial of service attacks on other apps. 

\subsection{Implementation choices to protect against active attacks from client apps}
\paragraph{Windowing manager-based attacks:} 
% \tarun{https://unix.stackexchange.com/questions/577086/how-do-i-detect-a-call-to-xorg-to-do-screenshots For X windowing manager, detect a call to Xorg to do screenshots and display to users the name of the ap that is doing. This will stop applications to intentionally doing anything malicious, provide them an incentive to secure their client end, and limit damage to users' privacy.}


In certain windowing systems, such as X11, there exist security risks associated with keylogging and screen capturing. When a user types in an application, other applications can retrieve keystrokes from the X server. The X server manages any graphics displayed on the screen and can be accessed by any application. However, in other windowing systems such as Wayland, access to keystrokes and graphics is limited to the corresponding application, providing higher security.

To mitigate these security concerns in the X11 windowing system, the \sysname architecture incorporates the Interceptor module, which intercepts plaintext before passing it to the X server and sends it directly to the GUI child process using shared memory. This ensures that the plaintext is not transmitted through the X server, preventing any application from accessing it.

As the X windowing server is a shared resource, all clients have equal access, which means any application can access \sysname's GUI graphically through screenshotting or screen recording. Currently, there is no way to prevent this. However, the Interceptor can monitor calls made to the window manager's screenshot API 'XGetImage' and notify the user whenever an app attempts to record the screen. To minimize the privacy harm to the user, a strong measure the Interceptor can take is to block all keyboard inputs and not let them pass whenever a screen record API is called, causing a denial of service.

An alternative approach to secure X-based attacks is to require the GUI process to pass plaintext directly to the display frame buffer, bypassing the X server. This prevents any application from scraping text from the display or capturing screenshots and recordings, as the X server has no access to the plaintext.

\paragraph{Run \sysname with as a different user} 

\sysname runs its Interceptor as a separate user with its own unique UID and GID. By running the Interceptor as a separate user, it can have its own set of permissions and access controls, which can help protect against potential attacks that exploit vulnerabilities in the user's system. 

One specific vulnerability that is addressed by running the \sysname processes as a different user is the possibility of an attacker using ptrace to attach to the process and dump the memory of the userspace GUI. Some distributions have \textit{ptrace\_scope} set to 0 by default, which allows any process under the same user to attach to any other process under the same user. This can be a significant security risk, as it enables an attacker to potentially gain access to sensitive information.



 \paragraph{Secure implementation ideas}
When implementing \sysname, it is crucial to consider the security risks that may be introduced during implementation to ensure its security.
The attacks based on implementation are out of the scope of this paper; however, we discuss the two most common implementation attacks that pose a high risk: shared object injection and python library substitution. Shared object injection involves an attacker setting the \textit{LD\_PRELOAD} environment variable to replace essential libraries with malicious ones. Python library substitution consists of an attacker overwriting userspace installed dependencies with malicious modules. This could result in the interception of sensitive information without any special permissions. One possible mitigation is bundling all dependencies together, ensuring all required libraries are included in a self-contained environment.
 
Also, the implementation of \sysname needs to ensure that private keys and decrypted messages are stored in a directory that is owned by the user that runs the Interceptor and has restricted permissions.

\paragraph{Key Management}

% A malicious package could overwrite the local cache of public keys and/or proxy the connection to the central Signal server. They could then replace all public keys of their own, and then intercept the encrypted keystrokes and decrypt them.
% Mitigations
% The cache should be protected with either file-system protections or encryption. The client should ship with a certificate store identifying the central Signal server and warn if the certificates do not match.

\sysname employs the signal protocol for encryption across multiple applications, allowing two users to communicate securely over different apps. In terms of key management, \sysname can use two options. Firstly, \sysname can generate a new public-private key pair for each user as it happens in the Signal protocol, and the sessions are updated across the applications. Alternatively, the client can maintain a different public-private key pair for every user for every app. However, the second approach offers no additional security benefits, as all the keys are stored in the same location on the client's machine, which can be a single point of failure.

On the other hand, the first approach does not pose any significant privacy risks as compared to the second approach. In the second approach, every client uploads their different public key for every app they use, which allows others to retrieve those keys to check if a user uses that app. This, in turn, could potentially reveal sensitive information to unauthorized parties. Therefore, we include the first approach of generating a new public-private key pair for each user in \sysname.

Moreover, by utilizing the same key bundle across different applications, \sysname simplifies the key management process and reduces the complexity of the system. A client in \sysname only needs to securely store the same key bundle as a signal protocol.

When a pair of users switch their communication from one app to another while using \sysname, the same session is used, and keys keep ratcheting as in the Signal protocol. This means the keys are updated and advanced every time a message is sent or received, ensuring the messages are encrypted with a fresh set of keys. This mechanism provides forward secrecy in the Signal protocol.

\tarun{Talk about key distribution and multi-device support.}



\subsection{Feasibility and Performance test}
We tested our prototype across a few sets of applications to determine their robustness. Our prototypes work for the following communication apps and websites: Gmail, Slack, Facebook, Microsoft Teams, and Discord. We also successfully tested our prototypes for google docs, where a user encrypts the sensitive part of the document before sharing it with another person. Only the recipient can decrypt the sensitive part of the document.

For complete coverage of all apps the MitM proxy needs to be extended to intercept all popular protocols such as HTTP2, HTTP3, sockets, and QUIC. It also accounts for different encodings that applications use to transmit their data. Future work is needed to identify the distribution of different protocols and encodings used by thousands of popular applications.


As shown in Table~\ref{tab:performance}, \sysname introduces two negligible delay overheads and one additional memory overhead. Once installed on the user's machine, \sysname continuously monitors the keyboard input file for encryption or decryption shortcuts. This process adds only [] milliseconds to each keystroke, which is imperceptible to the user. 

When encryption is initiated, every keystroke is encrypted in real-time, adding only [] additional milliseconds to XOR the character with the precomputed key stream. As metadata is not displayed, it can be computed in parallel, so users do not experience any delay in seeing the encrypted text.

After the user enables encryption, the MITM proxy process listens to all outgoing traffic from the target application, adding only a few milliseconds of delay to the outgoing traffic. This delay includes parsing the data, searching for ciphertext, and forwarding it.

While \sysname maintains a one-to-one mapping from plaintext to ciphertext, it adds metadata to each exchanged message, resulting in an increase of [] bytes in data size. This additional metadata needs to be stored by servers for each encrypted message exchange, and users need to transmit and receive more network data. The metadata is not visible to users in the GUI.


\input{table_performance}


The implementation of \sysname introduces two types of memory overhead: (1) users' devices need to store decrypted data, and (2) the application servers need to store additional \sysname metadata that is transmitted by the user. The extra metadata being transmitted is equivalent to the additional network data that the user will send or receive while transmitting the data encrypted through \sysname.

The amount of memory used to store decrypted text on the user's device will depend on how much data they encrypt using \sysname. Essentially, this overhead is proportional to the size of the data. Additionally, if users wish to do so, they can store backups of their data with symmetric encryption on other cloud storage services.

The extra metadata overhead comprises the following components in bytes: message version, ciphertext current version, ratchet key, ratchet key length, counter key, counter value, previous counter key, previous counter value, ciphertext key, ciphertext length, and MAC. The approximate total size of the metadata is $50 + \lfloor{\frac{\text{plaintext length}}{128}}\rfloor + 2\lfloor{\frac{\text{message number}}{128}}\rfloor$.


















% We will organize our description of the implementation by discussing a typical encryption process. First, the system is behaving normally. The user types the "encryption" shortcut, and a GUI appears. The user types the message: the plaintext is displayed in the GUI, and the ciphertext is displayed in the GUI or directly in the target application depending on the UI design. The user types the "encryption" shortcut again: after some finalizing by the system, the application has either a token which is read and changed by a background proxy or the entire Signal protocol message. The system returns to normal operation.

% This section describes our prototype implementation, not our intended final implementation.

% \subsection{Waiting for Initiation}
% Before the background daemon can actually perform useful work, it performs a bit of setup. The only argument given to the program is an absolute path to a /dev/input/ file; this file represents the input of the keyboard to monitor.
% \begin{enumerate}
%     \item The program opens the /dev/input/ file in a readonly nonblocking mode.
%     \item Using this file descriptor, the program employs Libevdev, a C library for interfacing with evdev (event device) devices, to create two structs: one representing the actual physical keyboard, and one representing the virtual keyboard through which the program will later send the encrypted message. Libevdev simply copies the layout of the physical keyboard to create a virtual clone. 
%     \item The program creates an new X window of no dimension using Xlib functionality. This window will later be used as a receiving location for a variety of X data.
% \end{enumerate}
% Once the program has performed these steps as well as various other initialization steps, a background daemon is in place and actively listening to the keyboard input file. The background daemon polls for changes on the input file, uses Libevdev to interpet the changes, and checks whether the input keypresses indicate the completion of the encryption or decryption shortcut. When the daemon detects the correct sequence of keystrokes, the program switches to the appropriate mode.

% \subsection{Encryption Enabled}
% When encryption is enabled, a few steps occur:
% \begin{enumerate}
%     \item The program uses the Libevdev library to grab exclusive access to the /dev/input file. If this grab is successful, no other application can read from the keyboard input file.
%     \item The program uses functionality in the Xlib library to record which application previously had input. This is necessary so that the daemon knows where to place the final message. The X window mentioned previously is used during this process.
%     \item The program begins the GUI. We choose to develop the GUI using the Tkinter Python library for Tcl/Tk. Tkinter's great advantage is that it is easily cross-platform.
%     \item The program does as much as possible to set up the encryption context. We use a modified version of Signal's libsignal-protocol-c C library for encryption. We preferred the C version because the overall program is very dependent upon system library calls, especially with regards to Libevdev.
%     \item The program begins an "encryption" thread for encrypting the characters and forwarding these characters to the application. We use a thread because, due to the nature of simulating key presses, it is necessary to introduce a delay between keypresses. This issue is described further in the following subsection.
% \end{enumerate}

% However, even though encryption is enabled, the program cannot actually encrypt yet. The user must first select the intended recipient. For this purpose, when the GUI starts, two windows appear:
% \begin{itemize}
%     \item A "main" window. This is the long-term window where the user will eventually be able to see the plaintext.
%     \item A "select recipient" window. This window is quickly populated with all available recipients. The daemon sends, via a Unix socket, the possible recipients. After selecting a recipient and clicking "confirm", this window disappears and the GUI forwards the selected recipient to the daemon.
% \end{itemize}

% Once the user selects a recipient and confirms the selection, the program moves to the "encrypting message" stage.

% \subsection{Encrypting the Message}
% When first entering this stage, the program performs a few additional preliminary steps:
% \begin{enumerate}
%     \item The main thread of the daemon uses the modified Signal C library to prepare the keys for this session. The Signal library (and the great majority of cryptography libraries) was designed around the idea that, when encrypting, the final message is complete and known. Since we want to make the "intermediate" ciphertext available to the user, we had to add a modified stream cipher version. To prepare to encrypt under this modified version, the main thread encrypts a few bytes of 0s.
%     \item The main thread returns the focus to the previously selected window under the "backspace" scheme.
% \end{enumerate}

% As the user types the plaintext message, a few steps occur inside the main thread for every keystroke:
% \begin{enumerate}
%     \item The main thread checks if the keystrokes complete a keyboard shortcut. If so, the system moves to the Finalizing Encryption stage.
%     \item The main thread interprets the evdev keystroke as an ASCII character, with some modifications to allow for arrow key movement.
%     \item The main thread immediately forwards this ASCII character to the GUI, and the GUI immediately updates its view of the plaintext.
%     \item The main thread also immediately forwards this ASCII character to the encryption thread.
% \end{enumerate}

% Meanwhile, the encryption thread performs these operations in a loop:
% \begin{enumerate}
%     \item The encryption thread waits to receive a new ASCII character.
%     \item The encryption thread then attempts to read as many ASCII characters as possible. Once there have been no new characters for a certain period of time, the thread continues with the next step.
%     \item The thread makes the requested modifications to its plaintext buffer.
%     \item If the recipient has been selected, the thread uses the prepared Signal keys to encrypt the new plaintext. As previously mentioned, the Signal library was not originally designed to continuously update the ciphertext based upon a changing plaintext, so we added functionality necessary to perform the following operations:
%     \begin{enumerate}
%         \item The library checks to make sure that its "one-time-pad", which was generated by encrypting a block of 0s, is long enough for the message.
%         \item If the pad is not long enough, the library encrypts a few additional blocks of 0s and appends these to the one-time-pad.
%         \item Now that the pad is long enough, the library performs a simple XOR with the plaintext and the one-time pad to create the ciphertext.
%     \end{enumerate}
%     \item Now that the message has been encrypted, the encryption thread encodes the message with Base64. This ensures that all characters are printable.
%     \item Finally, and under the "backspace" system, the encryption thread writes through the Libevdev Uinput virtual keyboard the necessary keystrokes to convert from the previous Base64 ciphertext message and the current Base64 ciphertext message. Under the "backspace" system, this first involves writing a sometimes large number of backspaces. After each keystroke, the thread waits for a very short period of time (currently 0.00125 seconds). This artificial delay is necessary because, otherwise, it is likely that the kernel's internal /dev/input ringbuffer will be overloaded, leading to lost keystrokes. In fact, it is this artificial delay which necessitated an encryption thread in the first place. Without a thread, the GUI has very poor performance, since the system may be outputting the keystrokes for the previous version of the ciphertext.
% \end{enumerate}

% Under the "backspace" system, the Base64 on screen is always in a "complete" state in terms of the Signal protocol, except when the encryption thread is updating the text. This means that a user could send the encrypted bytes without ending the encryption session with the encryption shortcut.

% The system will behave differently for the "overlay" and "proxy" versions.

% \subsection{Finalizing Encryption}
% When the main thread of the background daemon detects another encryption shortcut, it performs the necessary teardown:
% \begin{enumerate}
%     \item Under the "backspace" system, the main thread closes the connection with the encryption thread and waits for it to finish. This allows the encryption thread to finish updating the ciphertext before it returns.
%     \item Once the encryption thread has been closed, the background daemon adds the hash of the ciphertext and the plaintext to a local cache file. While currently rudimentary, this allows the user to later "decrypt" the ciphertext message. Without this, it is impossible for the sender to see what the message was.
%     \item The background daemon cleans up the Signal encryption context. In particular, the Signal keys are appropriately ratcheted, the one-time pad is zeroed out and freed, and the underlying cryptographic structures are freed.
%     \item The background daemon uses Libevdev to release its exclusive grab of the keyboard file, thus allowing other applications to resume reading from it.
%     \item The background daemon kills the GUI.
% \end{enumerate}

% \subsection{Return to Normal Operation}
% Now that everything has been cleaned up, the program returns to its original state of waiting for initialization.

% Backspace, Overlay, Mitmproxy versions

==> introduction.tex <==
\section{Introduction}

\tarun{Talk about the application of our E2EE. It is not for masses but for people in censored countries, organizations with sensitive date to keep them compliant.}

In the modern era of digital communication, secure and private communication is of utmost importance due to the frequent exchange of sensitive data. Transport Layer Security (TLS) is a widely used encryption protocol that provides security for data in transit. While TLS is an effective encryption protocol to \ks{the closing phrase is unclear} prevent user-to-server communication, it is insufficient for user-to-user communication as servers can see plaintext, leaving users vulnerable to interception. Therefore, there is an urgent need to provide end-to-end encryption (E2EE) for all user-to-user communication. E2EE encrypts the message contents from the sender's device, and only the intended recipient can decrypt the message, making it difficult for anyone else to intercept, read or modify it. 

Although E2EE is a viable solution, the issue lies in the fact that applications, not users, decide when to implement E2EE. Currently, most popular applications, such as Email, Slack, Microsoft Teams, and Discord, still use TLS, making it difficult for users to secure their communication. Moreover, even when the applications implement E2EE, their client apps have access to plaintext, which could lead to unintended leakage due to bugs or intentional breaches. Furthermore, users often do not trust E2EE applications~\cite{abu2018exploring} as they cannot visibly distinguish between plaintext communication, TLS encryption, and E2EE. Because of the lack of encryption visibility, users rely on the app developer's words to understand the secure data from their app, which has conflicting interests.
\ks{Closing sentence unclear.}

We design a Secure Input driver (\sid) and Secure extension for the Input driver (\seid) that (1) allows users to request encryption on any textbox on any application even if an application doesn't support it and (2) makes it easier for developers to support E2EE for their applications using our APIs in any language. SID is designed as a kernel module, which allows isolation from user-space vulnerabilities and easy distribution to the user's machine in the long term. In contrast, SEID is designed as a user-space application allowing it to be compiled for any platform with necessary libraries and dependencies. SEID is a better choice in the short term as user space development is faster and simpler than kernel module development, with fewer memory allocation constraints and more straightforward debugging. Furthermore, SIED's isolation from the kernel ensures that early-stage adoption does not compromise the entire system due to code crashes or vulnerabilities. Both design (1) supports application independent encrypt to support all kinds of applications, (2) prevent plaintext access from non-root client applications, and (3) enhances trust through translucency. 
\ks{I don't really understand how SID and SEID differ from this paragraph.}

Our design monitors keystrokes directly through the keyboard driver to provide application-independent and scalable encryption. When a user press shortcut to enable encryption mode, our system encrypts everything before passing the text from the keyboard driver to the X11 windowing, which is responsible for passing the keypresses to applications. \seid shows users a secure \sysname\_GUI that displays the plaintext input and live encrypted text in the application GUI character by character. It adds metadata using a network proxy before transmission over the Internet., which it setup and activated after a user enables encryption.

% We present three variations of \seid, each providing a different user experience. The first variation, \ls, shows users a secure GUI that displays the plaintext input and live encrypted text along with metadata in the application GUI character by character. The second variation, \ds, also displays the plaintext input in a secure GUI but shows seemingly encrypted random junk characters in the application GUI, with the encrypted text and metadata being added by a network proxy before transmission over the Internet. Finally, the third variation, \os, overlays the entire screen and allows users to enter plaintext, which is then encrypted and automatically pasted into the application GUI after the user finish encryption.
\ks{These explanations need improving. The names are cryptic and }


Contributions
\begin{enumerate}
    % \item Present an E2EE system with visible encryption that could lead to increased trust in the user and can be used by researchers to confirm this hypothesis in future user studies.
    % \item Design an E2EE architecture with better security properties, such as no client app access to plaintext and visible encryption that could lead to increased trust in the user.
    % \item we present 3 variants of design that provide the same amount of security but different UX. Usability researchers can test these systems to study the UX for better adoptability of these systems. These prototyped are developed under constraints of current OS design to allow testing of deployable and more realistic UX.


\item Improved E2EE Architecture: The paper proposes an end-to-end encryption (E2EE) architecture that offers better security properties. The proposed design eliminates the client app's access to plaintext, ensuring that the data remains secure even if the client app is compromised. Additionally, the architecture incorporates visible encryption, which makes it easier for users to understand that their data is being encrypted and provides them with greater confidence in the system's security. 
\ks{I think the terms improved and better are difficult to include because it doesn't answer the question of better than what?}
\ks{I think two contributions here should be split into two items: the application has no access to plaintext, and encryption is visible.}
\ks{Isn't the application-independent approach a contribution? Or maybe not, since others have provided it?}

\item Prototyped Designs for Realistic Testing: To ensure the practicality and feasibility of the proposed E2EE architecture, the paper presents three variants of the design, each with the same level of security but different user experiences. These prototypes are developed within the constraints of current operating system (OS) designs, making them more realistic and deployable. Usability researchers can test these prototypes to evaluate the user experience and study their adoptability by end-users. This testing can help identify any usability issues and provide insights into how to improve the design for greater user acceptance.
\ks{I think this will be a tough sell to tier 1 with no user study of the basic approaches. Usability people will wonder why you didn't do user-centric design from the start.}

\end{enumerate}

\ks{Another aspect of the system is the granularity. Are all other E2EE systems an all-or-nothing approach where entire message or file is encrypted? We allow fine-grained encryption where a document, email, message can have specific sensitive data items encrypted while the rest is visible to the server. Is this a plus?}

% \subsection{Motivation}

% Most of the user-to-user communication still happens o


% An Empirical Study of Insecure Communication in Android Apps
% http://gossip.yyjess.com/wp-content/uploads/2021/04/WCNE2016Zhang.pdf

% \subsection{Why E2EE?}

% End-to-end encryption (E2EE) and Transport Layer Security (TLS) are both important security mechanisms used to protect data during transmission, but they serve different purposes and have different strengths and weaknesses. Here are some reasons why E2EE is considered better than TLS in some contexts:

% Complete encryption: E2EE provides complete encryption of the data from the sender's device to the recipient's device, meaning that the messaging service provider and any intermediaries cannot access the content of the message. In contrast, TLS provides encryption between the client (e.g., web browser) and server, but the data may be decrypted at the server and accessed by the messaging service provider.

% Protection against server attacks: E2EE protects against attacks on the messaging service provider's servers, as the encrypted data is useless to anyone who does not have the decryption key. In contrast, with TLS, if the server is hacked, the encrypted data may be accessed and compromised.

% Stronger security: E2EE uses stronger encryption algorithms and key exchange protocols, which can make it more difficult for attackers to intercept or access the data.

% Greater privacy: E2EE provides greater privacy for users, as the messaging service provider cannot access the content of the messages, meaning that the data cannot be used for advertising or other purposes.

% However, it's worth noting that TLS is still important for securing data in transit between the client and server, and it provides additional security measures such as server authentication and data integrity checks. Additionally, E2EE can have limitations such as the need for users to manage encryption keys, which can be cumbersome for some users. Overall, the choice of security mechanism will depend on the specific use case and the level of security and privacy required.


% end-to-end encryption is important

% Privacy: End-to-end encryption ensures that only the intended recipient can read the message, making it difficult for others to intercept or view the message.

% Security: End-to-end encryption prevents third parties from tampering with the message or altering its content during transmission.

% Legal compliance: End-to-end encryption can help organizations to comply with data privacy and security regulations, as it ensures that personal data is protected.

% \subsubsection{Why TLS is insufficient?}
% TLS uses PKI certificates to authenticate parties communicating with each other as well as encrypting the communication session. The PKI security is based on the trust of Certificate authorities. Previous research shows the instances of notorious behavior of CAs and their compromises, which breaks the TLS protocol's security. Using E2EE with manual or automated key verification (our suggested protocols) reduces trust in unknown third parties like CAs or servers. And with the current proposals of automatic key verification, all the E2EE key authentication is transparent from users.

% There also exist TLS middleboxes on the Internet ~\cite{lee2019matls}. Some of them are legitimate, some are malicious, and they have access to plaintext for all the communication going through them. Users/ Application developers have no control over it, and they cannot do anything to prevent eavesdropping/packet modification from these TLS proxies on any part of the communication.

% As of now, users trust the webserver for most of the communication. Even it's not only about trust on the web service servers; users also need to trust the third parties with whom webservices share their key TLS private keys. Most of the third parties should be hosting providers or CDNs; however, users' communication privacy depends on the chain of trust from the server. And users have no control over the TLS keys at the server end. Previous research shows that over 76\% of all organizations share at least one of their private keys with a third-party hosting provider. As a result, compromising the most popular hosting provider could provide access to the private keys for 60\% of the domains in the Alexa top-1K ~\cite{cangialosi2016measurement}. The overall communication security is dependent on the web server's communication access policies and their TLS key delegation policies.




% Our idea is to provide E2EE to any application in a scalable manner. Therefore we require a triggering mechanism from the user (which data to encrypt and to whom). This is scalable to all the applications and all the data types (The data type can be text, image, or file). We intercept the system call and encrypt it before the application receives the data. 


% \subsection{Contribution}

% PROTOCOL IDEA
% Design an E2EE that any application uses easily with a minimalistic line of code for any application's text field. It is going to be transparent to the user. The user will be displayed a notification popup on the window screen in the corner and stays until the user types in the E2EE text field.
% A user can use the protocol for any content even if an application does not support encryption. When encryption initiation is trigger by the user. When a user triggers the encryption, a popup on the screen is displayed until the user triggers the encryption stop. And then the user is popped up with the user to which encrypt. 
% Do two user studies for this protocol— one for developers and the other for users to see how feasible this design is. 


==> system_and_adversary_model_old.tex <==
\subsection{System and Adversary Model}

In our system, clients communicate through centralized client/server architectures. Peer-to-peer communication, where users communicate directly, is out of the scope of this paper. 
\ks{Are there peer-to-peer systems offering E2EE? We might want to have a short paragraph in RW about this. Perhaps none are used very much, so our goal is to design a system to add E2EE to existing apps since users won't migrate to P2P apps for reasons we've already established. That gives us a reason why we chose not to explore P2P systems. It is another way to circumvent trusting companies and perhaps adopting those apps is easier than adopting InfoGuard.}
\tarun{Even for the P2P apps, doesn't the user need to trust the client end? Perhaps you are talking about achieving the current level of E2EE where we just want to protect messages from the server. Regardless, I think \sysname would also work for P2P. It does not matter what protocol they use to relay the messages. We just replace the plaintext with encrypted text at the application layer, and the client app can relay however they want. From the implementation point of view, we will just need to include the protocol in mitm proxy to intercept and append metadata. }

\textbf{Clients}: The software applications that enable users to communicate with each other over the internet and are installed on their devices. Examples of such clients include Slack, Outlook, or webpages accessed through a web browser.

\textbf{Servers}: The intermediaries that facilitate communication between clients. They can be messaging, email, or any other server supporting client-to-client communication.


\textbf{Input device driver}: An input device driver is a software component in the OS that enables communication between the OS and the input devices, such as a keyboard. The driver ensures the device's proper functioning by translating signals the input device sends into a format that OS can understand. 

% \subsection{Definitions and Assumptions}

Client-to-client communication involves the exchange of messages between two or more users over the Internet. When a user wants to send a message to another user, they first enter it using an input device such as a keyboard. The input device driver process and passes the message to the windowing manager, such as X11 or Wayland. Then, the plaintext input is retrieved by the corresponding application. The application encrypts the message using TLS, and the network interface sends it over the Internet to the application's server. The server decrypts the message, re-encrypts using the TLS connection for the recipient, and delivers it to the recipient. Upon receiving the message, the recipient's device receives and decrypts it, allowing the recipient to read it.

Some applications support E2EE, such as Signal. After receiving the user's input from the windowing manager, these applications encrypt the input with a key shared with the recipient before it is encrypted for transmission over TLS to ensure the server cannot access the user's data when they decrypt the TLS transmission.


\paragraph{Adversary model}
Adversary \A is an active global attacker that controls an application server and has plaintext access to all messages and metadata flowing through the server. 
\A also controls client applications having user (non-privileged) access.
%the usual user-level privileges (not sudo or root access).

The adversary \AB is an active global attacker that controls an application server and has plaintext access to all messages and metadata flowing through the server. \AB also passively observes all the text received or sent by the client application.

We consider two different threat models based on who is attempting to secure an input text. In the first scenario, when a user attempts to secure an input text, we assume an adversary \A. In the second scenario, when an application attempts to secure an input text, we assume adversary \AB. To achieve text security, an application must explicitly call our API, so it is infeasible to prevent access from an active attack by the client application.\\
If both the user and the application attempt to secure an input text, we assume a stronger adversary \ie \A. 
\ks{Not sure about terms text, input text, text security. Is this like texting? Can we refer to data? Is the issue that we only focus on keyboard input for now?}

The adversary could be (1) law enforcement or an oppressive regime coercing an application or (2) hackers compromising an application. 
The adversary's goal is to compromise message confidentiality and integrity to be able to read and modify users' messages.
\ks{I'm not sure of A2 assumptions for a scenario 1. If the server is being coerced, it would probably force app to disable developer encryption to capture the data. I'm not sure the two scenarios are coherent together.}
\tarun{Agree! However it is not completely contradictory. In this paragraph, we are giving a few examples who can be the above adversaries. Even A2 is possible for scenario 1, where the companies are willing to have a passive backdoor code in their app that share data with govt, however executing an active attack that is detectable could be a risk for companies and govt too. Therefore, claiming that the govt or companies prefer to listen passively and prevent against that is a feasible solution. One point to note is an app can always disable E2EE, however user will know that data is not E2EE as they will not see a separate GUI. Therefore they need to create a fake GUi to get users' trust to get their sensitive data.}
\ks{That is an interesting attack. This attack should be mentioned in discussion section about potential vulnerabilities with this approach. Can we think of others?}



% \ks{I wonder if one way to talk about this is to assume we are not talking about peer-to-peer systems where users communicate directly. Instead, we focus on the common architecture where users communicate through centralized client/server architectures. Is this accurate?}



==> table_performance.tex <==
\begin{table}
	\centering
	\caption{Performance analysis}
	\label{tab:performance}
 
	\begin{tabular}{|p{3cm} |p{3cm} |c|}
         \hline
        \multicolumn{2}{|c|}{Overhead} & Value \\
         \hline
        Delay while waiting & & \\
        \hline

          Delay due to encryption & key press -> GUI & \\
        \cline{2-3}
                                & MITM proxy & \\

        \hline
        bytes per message & user's GUI & 0 \\
        \cline{2-3}
                        & to Server & \\
        \hline
      



	\end{tabular}
	
	% \vspace{3mm}
    
	% $\ddagger$~ = detects with $0.999$ probability\\
% 	\detects~detects the attack, \partialp~sometimes prevents the attack \\
\end{table}


==> todolist.tex <==
\section{TODO Items}

\begin{enumerate}
    \item Title options: \\
    User-Controlled Encryption \\
    User-Controlled Application-Independent Encryption \\

   \item System names to consider:\\
   System-Wide Input Security (SWIS),
    Application-Independent Input Encryption (AIIE)
    AnyInput Encryption System (AIES)
    Secure Input Anywhere System (SIAS)
    InputGuard (IG)
    SecureInput (SI)
    InputArmor (IA)
    Redacto, Blackout, Cover, Conceal, Obscure, Hide, Hidden, Protect, Guard, Shield, Private <some variation of these words>
    SafeGuard, TextGuard, InfoGuard, DataGuard
    MessageShield, Message Guardian (MG), \\
    
    \item Who are the other co-authors or acks that will be on the paper, especially the undergraduate contributors? Should we be involving any of them now in the writing/review process?\\
    \tarun{Justin would be a co-author. Austin has been working long with UI and some performance analysis numbers. As a sophomore, it took him longer to contribute, but he is on this project for a year now. Not sure, if he should be an author. Any suggestions/thoughts?}
    Co-authors: Justin Hales,
    Ack: Austin Cook, Jonathan Chelius? ,
    So for Justin should we reach out and share paper, invite him to help review now? Any task to give him if he has time?\\
    \tarun{I am not sure if he can help with the writing, but could be helpful doing proofreading. We can reach out to him and let him know that we are planning to submit the paper on May 4th and ask if he has time next week to review it and help us improve the writing of the paper.}\\
    \ks{Is Alden now working on this paper and could be acked, or is his contribution for the future? Did Scott or Joshua look at this and give feedback? I think they have done some of our papers but I haven't kept track to ack them when it is published.}
    \tarun{I also propose adding Austin as the author. He might not have significantly contributed to one part of the project, but now I realize he helped with a lot of small things here and there. He helped with app analysis, helped with reddit codes, GUI, and implementation bugs. Furthermore, he is planning to work next semester too where he can help make changes if needed during revison. I believe this is more than enough contribution to be an Author. And I propose to Ack Alden and Jonathan. }
    
    \item Should we include the developer API in this paper? 
    \ks{I vote no. It runs counter to main theme of user-controlled encryption. It raises the reviewer attack surface and I don't think it is needed to get the paper published. Maybe mention it as future work. But what are the good reasons to include it?}
    \tarun{I am in favor of adding it to the paper. However, open to adding it to the discussion after we discuss this on-call or in person. It allows applications to achieve E2EE easily where their client app does not have access to plain text. Honest applications can quickly include this E2EE for their inputs to secure users against their client-side vulnerabilities and gain users trust. For the developer API, we trust the app and assume it does not perform an active attack. I think developers' API would be nice to include as it's a high-impact low hanging fruit. I updated the threat model section to include a different threat model for that. I am okay adding it in the discussion section if you strongly prefer that or if you think there are issues with it. We can take a call on this after we discuss this on the call.}
    \ks{See my questions in threat model section. I'm willing to try it, but let's see if we can include all of this in the paper length limit. }
    \\

    \item \ks{I've been doing some reading about the differences between an architecture design and a systems design. Which do we have? Definitely a systems design, but is there value in having both? }

    \item \ks{I'm leaning we list encrypted search as future work since we didn't build it and don't have a contribution in that space. Application-level searching will continue to work on plaintext portions of the data. Searching sensitive data may be a useful feature to explore. Will leaving it for future work be a reason for rejection? I don't think so. }
    \tarun{Agree! Will move that to the discussion section. According to my understanding, whenever I see E2EE papers they are concerned about how it is gonna affect basic features like searching. So, I would like to comment on this for sure, but the discussion section should be okay.}
    \ks{Sounds good. We will include this as room permits, and it could be brief in discussion.}
    \item{Is the recent paper I found related to this work discussed?} \tarun{Not yet. Will add.}
    \item {How do we characterize the reddit users? Is it experts? It sounds like it has novices that are asking questions. How to we explain the implication of the results if we can't characterize the users? Idea: We study this because it is real people asking questions and providing advice in the real world on the topic we are interested in. This is different than recruiting people to interview on a subject, which also has its own limitations.} 
    \item I had another idea for a point to make in the paper. We have language about \sysname circumventing censorship in countries that ban certain apps. I think our approach raises the bar on censorship. There is no app to ban based on well-known ports or protocol signatures that can be blocked. It would require scanning the application data for encrypted text and blocking individual messages. This could not be done for TLS transmission, but could work on unencrypted protocols. But now the censor has to scan the application data actively and cannot block based on meta properties. Is this worth a point in the discussion?
    \tarun{Yes!}
    \item Some place in the paper we should emphasize the novelty of this application-independent approach. Very different than the status quo and something research should explore. We show it is feasible and worth future study.
    \tarun{Yes! I would like it to bring it in the Introduction. However, we will need to be careful as we are not the first one. Scotts' MessageGuard, Mimesis Aegis are some application independent encryptions too. Two unique properties are: (1) first desktop application-independent approach that also works outside of browser. (2) no need to update the system for application-specific GUIs.}
\end{enumerate}

